Auto-Tag: Tagging-Data-By-Example in Data Lakes

As data lakes become increasingly popular in large enterprises today, there is a growing need to tag or classify data assets (e.g., files and databases) in data lakes with additional metadata (e.g., semantic column-types), as the inferred metadata can enable a range of downstream applications like data governance (e.g., GDPR compliance), and dataset search. Given the sheer size of today's enterprise data lakes with petabytes of data and millions of data assets, it is imperative that data assets can be ``auto-tagged'', using lightweight inference algorithms and minimal user input. In this work, we develop Auto-Tag, a corpus-driven approach that automates data-tagging of \textit{custom} data types in enterprise data lakes. Using Auto-Tag, users only need to provide \textit{one} example column to demonstrate the desired data-type to tag. Leveraging an index structure built offline using a lightweight scan of the data lake, which is analogous to pre-training in machine learning, Auto-Tag can infer suitable data patterns to best ``describe'' the underlying ``domain'' of the given column at an interactive speed, which can then be used to tag additional data of the same ``type'' in data lakes. The Auto-Tag approach can adapt to custom data-types, and is shown to be both accurate and efficient. Part of Auto-Tag ships as a ``custom-classification'' feature in a cloud-based data governance and catalog solution \textit{Azure Purview}.

==> architecture.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{System Architecture}

TBD



==> auto-validate-horizontal.tex <==
%!TEX root = main.tex
%\vspace{-2mm}
\section{Auto-Validate (Horizontal Cuts)}
\label{sec:horizontal-cuts}
So far we assumed the query column $C$
to be ``clean'' with homogeneous
values drawn from the same domain 
(as they are typically generated by the same program).
While this is generally true, we observe that many
columns can have ad-hoc special values  
(e.g., denoting null/empty-values)
not following the general pattern of normal values in $C$,
as shown in the example columns in Figure~\ref{fig:example-nulls}.

\begin{figure}
\vspace{-6mm}
        \centering
        \includegraphics[width=0.5\textwidth]{figures/example-nulls.png}
\caption{Example ad-hoc special values (in red boxes)
not observing patterns of other values in the column.}
\label{fig:example-nulls}
\end{figure}



We note that examples like these are not uncommon -- even for
machine-generated data, there can be a special 
branch of logic in the program
(think of \val{if-else}/\val{try-except}) that
 handles special corner cases (e.g., nulls),
and produces ad-hoc special values 
that would not follow the general pattern of ``normal'' values in the column.
We henceforth refer to these as \textit{non-conforming values}.

Recall that in FMDV, by assuming that the query column $C$ has
homogeneous values, we select patterns
from $\mathbf{H}(C) = \cap_{v \in C}{\mathbf{P}(v)}$, 
or the intersection of patterns for all values  $v \in C$.
Such an assumption does not hold 
for columns in Figure~\ref{fig:example-nulls},
yielding an empty $\mathbf{H}(C)$ and
no feasible solution if we were to use FMDV.

We thus consider a variant of \sj with ``horizontal
cuts'', meaning that we can ``cut out'' a small fraction
of non-conforming values in 
$C$ (which is identical to making patterns tolerate
a small fraction of non-conforming values). 
We use a \textit{tolerance parameter}
$\theta$ to control the maximum allowed fraction of 
non-conforming values that can be cut out (e.g., 1\%, 5\%, etc.).

The corresponding optimization problem, termed
FMDV-H, is defined as follows:

\begin{align}
\hspace{-1cm} \text{(FMDV-H)}~~\min_{h}~& \text{FPR}_\mathbf{T}(h)   \label{eqn:fmdvh_obj} \\ 
 \mbox{s.t.} ~~ & h \in \cup_{v\in C}{\mathbf{P}(v) \setminus \text{``.*''}} \label{eqn:fmdvh_h} \\
&  \text{FPR}_\mathbf{T}(h) \leq r \label{eqn:fmdvh_fpr} \\
 & \text{Cov}_\mathbf{T}(h) \geq m \label{eqn:fmdvh_cov} \\
 & |\{ v | v \in C, h \in \mathbf{P}(v) \}| \geq (1-\theta) |C| \label{eqn:fmdvh_tolerance}
\end{align}

Like before, our objective function is to 
minimize FPR in Equation~\eqref{eqn:fmdvh_obj}.
Equation~\eqref{eqn:fmdvh_h} shows that the 
hypothesis pattern $h$ is drawn from
the union of possible patterns for all $v \in C$.
%(as opposed to $\mathbf{H}(C)$ in FMDV that uses intersection).
The FPR and Coverage requirements in
Equation~\eqref{eqn:fmdvh_fpr} and
Equation~\eqref{eqn:fmdvh_cov} are 
the same as the basic FMDV.
Finally Equation~\eqref{eqn:fmdvh_tolerance} requires
that the selected $h$ has to match at least 
$(1-\theta)$ fraction of values in $C$, where $\theta$ 
is the tolerance parameter above (the remaining
 $\theta$ fraction can be considered as non-conforming 
values that are cut out).

%revised
\iftoggle{fullversion}
{
\begin{example}
\label{ex:fmdvh}
Consider the leftmost column $C$ in Figure~\ref{fig:example-nulls}.
Using FMDV-H above, we determine that the pattern $h=$
``\val{<digit>+,<digit>+,<digit>+,<digit>+,<digit>+}''
to be a valid solution, as it meets the FPR and coverage
requirements based on an analysis of $\mathbf{T}$.
Furthermore $h$ is consistent with 99\% of values in $C$
(the remaining 1\% non-conforming value
is the ``\val{-}'' marked in a red box), thus also meeting
the requirement in Equation~\eqref{eqn:fmdvh_tolerance}.
\end{example}
}%iftoggle fullversion

\begin{theorem}
\label{thm:fmdvh}
The decision version of FMDV-H is NP-hard.
\end{theorem}

For arbitrary $\theta$ and generalization hierarchy,
we can show that deciding whether there is a feasible 
solution to FMDV-H is NP-hard (let alone minimizing FPR), using a reduction
from independent set~\cite{karp1985fast}.
% (e.g., by
%modeling each $v \in C$ as a vertex in a graph,
%and connecting two vertices if their corresponding
%values have no common generalized patterns
%except the trivial pattern \val{.*}).

While FMDV-H is hard in general, in practice because
the patterns of non-conforming values often
do not intersect with those of ``normal'' values,
%revised
\iftoggle{fullversion}
{
(as in Example~\ref{ex:fmdvh}),
}
 they create 
easier instances of FMDV-H for us to solve.
Leveraging this observation, in this work 
we optimize FMDV-H greedily, by cutting out
values whose patterns do not intersect
with most others in $C$.
We can then find the optimal pattern for the
remaining conforming values in FMDV-H 
using FMDV.


\textbf{Distributional test of non-conforming values.}
Given a pattern $h$ inferred from the
``training data'' $C$ using FMDV-H, and given the
data $C'$ arriving in the future, we need to
to determine whether the fraction of non-conforming
values in $C'$ has changed significantly from $C$.

Specifically, at ``training'' time,
we can calculate the fraction of values in $C$ not 
conforming to $h$, denoted as $\theta_{C}(h) 
= \frac{|\{ v | v \in C, h \notin \mathbf{P}(v) \}|}{|C|}$.
At ``testing'' time, we also compute the fraction of 
values in $C'$ not 
matching $h$, denoted as $\theta_{C'}(h)$.


%\revised
\iftoggle{fullversion}
{
A naive approach to validate $C'$ is to trigger alarms
if $\theta_{C'}(h)$ is greater than $\theta_{C}(h)$.
This however, is prone to false-positives.
Imagine a scenario where we compute the non-conforming ratio
$\theta_{C}(h)$ on training data $C$ to be 0.1\%. 
Suppose on $C'$ we find $\theta_{C'}(h)$ to be 0.11\%.
Raising alarms would likely be false-positives.
However, if $\theta_{C'}(h)$ is substantially higher, say at 
5\% or even 50\%, intuitively it becomes an issue
that we should report. (The special
case where no value in $C'$ matches $h$
has the extreme $\theta_{C'}(h)=$ 100\%).

To reason about it formally, we 
model the process of drawing a conforming value
vs. a non-conforming value in
$C$ and $C'$, as sampling from two binomial distributions.
We then perform a form of statistical hypothesis test called 
\textit{two-sample homogeneity test},
to determine whether the fraction of non-conforming values
has changed significantly,
using $\theta_{C}(h)$, $\theta_{C'}(h)$,
and their respective sample sizes $|C|$ and $|C'|$.

Here, the null-hypothesis $H_0$ states that the
two underlying binomial distributions are the same;
whereas $H_1$ states that the reverse is true. 
We use \textit{Fischer's exact test}~\cite{agresti1992survey}
and \textit{Pearson's Chi-Squared test}~\cite{kanji2006} with
Yates correction for this purpose, both of which are suitable tests
in this setting.
We report $C'$ as an issue if the divergence from $C$ 
is so strong (e.g., $\theta_{C}(h) =$ 0.1\% and
$\theta_{C'}(h) =$ 50\%) such that the null hypothesis can be rejected.


We omit details of these two
statistical tests in the interest of space. 
In practice we find both to perform well, with 
little difference in terms of validation quality in our experiments.
}%iftoggle
{
We model the process of drawing a conforming value
vs. a non-conforming value in
$C$ and $C'$, as sampling from two binomial distributions.
We then perform a form of statistical hypothesis test called 
\textit{two-sample homogeneity test}, specifically using
\textit{Fischer's exact test}~\cite{agresti1992survey}
and \textit{Pearson's Chi-Squared test}~\cite{kanji2006} with
Yates correction. We report $C'$ as an issue if the divergence from $C$ 
is strong.
We omit details of these statistical tests in the interest of space. 
In practice we find both to perform well, with 
little difference in terms of quality in our experiments.
}% else iftoggle



\revised{
\textbf{Time Complexity.}
Overall, the time complexity of the offline step is 
$\mathcal{O}(|\mathbf{T}| |\mathbf{P}(D)|)$,
which comes from scanning each column $D$ in
$\mathbf{T}$ and enumerating its possible patterns. 
Note that because we use vertical-cuts to handle
data domains with complex patterns (i.e., long token sequences),
we can constrain $\mathbf{P}(D)$ 
effectively by limiting the max number of tokens in $D$ 
(e.g., limiting max token size to 13 produces would upper-bound
$|\mathbf{P}(D)|$ to 500),
yet vertical-cuts can still handle the complex patterns
without loss of precision/recall.

In the online step, the complexity of the most involved
FMDV-VH variant is $\mathcal{O}(|\mathbf{P}(v)| |C| t(C)^2)$,
where $t(C)$ is the max number of tokens in query column $C$.
Empirically we find this to be less than 100ms on average,
as we will report in the experiment section.
}

%https://en.wikipedia.org/wiki/Binomial_proportion_confidence_interval
%Based on the Central Limit Theorem,
%we reject $H_0$ if 
%\begin{equation}
%\label{eqn:hypothesis-test}
%\theta_{C'}(h) > \theta_{C}(h) + z \sqrt{\frac{\theta_{C}(h) (1 - \theta_{C}(h)) }{|C|}}
%\end{equation}
%We use $z_{0.05}$ = 1.96  for a 95\% confidence interval,
%and consider the validation to fail if 
%the null-hypothesis is rejected. 

%Many statistical tests are possible here
%(e.g., Chi-Squared and Fisher's tests)










==> auto-validate-vertical.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Auto-Validate (Vertical Cuts)}
\label{sec:vertical-cuts}

So far we only discussed the basic-version of
\sj. We now describe formulations that handle
more complex and real situations: (1) \textit{composite} structures
in query columns (this section); 
and (2) ``dirty'' values in query columns that violate
the homogeneity assumption (Section~\ref{sec:horizontal-cuts}).



Figure~\ref{fig:example-split} shows a real
column with composite structures 
that is concatenated from \textit{atomic domains}. Intuitively, 
we can see that it consists of at least 4
``sub-domains'', a floating-number (``\val{0.1}''),
followed by two time-stamps, 
followed by a status message (``\val{OnBooking}'').
We observe that such columns are common
in machine-generated data in the data-lake, where 
many are complex with over 10 sub-domains.


Such complex columns pose both quality and
scalability challenges. The first is in terms of quality --
if we were to directly test complex
patterns against $\mathbf{T}$ like in FMDV, we may not be
able to see many exact matches in $\mathbf{T}$, 
because the complex patterns in $C$ may be concatenated 
in ad-hoc ways and are
sparsely represented in $\mathbf{T}$.
As a result, we would fail to find
any feasible solution to FMDV, 
because of the coverage requirement in 
Equation~\eqref{eqn:fmdv_cov}.

\revised
{
The second challenge of these complex columns is scalability --
as a column $C$ become ``wider'' with
more tokens/segments, the space of possible patterns $\mathbf{P}(C)$
 that we will have to enumerate
grows exponentially in the number of tokens.
This is an issue both at online query time
for query column $C$, as well as
at offline indexing time to enumerate 
$\mathbf{P}(D)$ for data column $D \in \mathbf{T}$ --
recall that the date-time example in 
Figure~\ref{fig:generalization} already produces
over 3 billion patterns;  for the column in
Figure~\ref{fig:example-split} the
space of patterns is only going to be 
impractically large to enumerate. 
As discussed in Section~\ref{sec:architecture},
we have to omit wide columns with
more than $\tau$ tokens from 
offline indexing to make pattern enumeration
tractable. We will show that the proposed 
vertical-cut algorithm
can ``compensate'' such omission without affecting result quality.
}

\revised{
A natural approach to complex query column $C$
is to vertically ``cut'' it into
sub-columns (like shown in  
Figure~\ref{fig:example-split}). Patterns for
each sub-column can then be generated in turn using FMDV.
The benefit of this divide-and-conquer
approach is that each sub-domain
is likely well-represented in $\mathbf{T}$,
allowing FMDV to make reliable predictions using $\mathbf{T}$.
Furthermore, the cost of pattern-enumeration becomes 
significantly smaller, as each sub-domain requires separate
enumeration.
}

Specifically, we first use a lexer to tokenize each $v \in C$
into coarse-grained token-class (\val{<symbol>}, 
\val{<num>}, \val{<letter>}), by scanning each $v$
from left to right and ``growing'' each token until 
a character of a different class is encountered. 
In the example of Figure~\ref{fig:example-split},
for each row we would generate an identical token-sequence
``\val{[<num>|<num>/<num>/<num> <num>:<num>:<num>|} \ldots \val{|<letter>]}''.

We then perform multi-sequence alignment 
(MSA)~\cite{carrillo1988multiple}
for all token sequences, before actually performing vertical-cuts.
Recall that the goal of MSA is to find optimal 
alignment across all input sequences 
(using objective functions such as 
sum-of-pair scores~\cite{just2001computational}).
Since MSA is NP-hard in 
general~\cite{just2001computational}, we follow
a standard approach to greedily align one additional sequence at a time.
We note that for homogeneous machine-generated 
data, this often solves MSA optimally.


\begin{example}
\label{ex:align}
For the column in Figure~\ref{fig:example-split},
because each value $v \in C$ has an identical token-sequence
with 29 tokens:
``\val{[<num>|<num>/<num>/<num> 
<num>:<num>:<num>|} \ldots \val{|<letter>]}'',
the aligned sequence using MSA can be
produced trivially as just the input sequence also with 29 tokens (with no gaps).
\end{example}


\begin{figure}[t]
\vspace{-14mm}
        \centering
        \includegraphics[width=0.45\textwidth]{figures/example-split.png}
\caption{Example columns with composite domains.}
\label{fig:example-split}
\end{figure}


After alignment, characters in each $v \in C$ would map to
the aligned sequence of length $n$
(e.g., ``\val{0.1}'' maps to the first \val{<num>} in the aligned
token sequence,
``\val{02}'' maps to the second \val{<num>}, etc.).
%we produce a sequence of tokens $S_i$ of same length $n$,
%written as $S_i = [t^i_1, t^i_2, \ldots, t^i_n]$, where each $t^i_j$ is
%a token at the $j$-th position of value $v_i$.
Recall that our goal is to vertically split the $n$ tokens 
into $m$ segments, so that values mapped to
each segment would correspond to a sub-domain as determined by FMDV.
We define an $m$-segmentation of $C$ as follows.

\begin{definition}
\label{def:segmentation}
Given a column $C$ with $n$ aligned tokens,
define $C[s, e]$ as a segment of $C$ that starts from token position 
$s$ and ends at position $e$, with $s, e \in [n]$.
An $m$-segmentation of $C$, 
is a list of $m$ such segments that
collectively cover $C$, defined as:
$(C[s_1, e_1], C[s_2, e_2],$ $\ldots$ $C[s_m, e_m])$,
where $s_1 = 1, e_m = n$, and $s_{i+1} = e_i + 1~\forall i \in [m]$.
We write $C[s_i, e_i]$ as $C_i$ for short,
and an $m$-segmentation as 
$(C_i : i \in [m])$ for short. 
\end{definition}

\revised{
Note that each $C_i$ can be seen just like a regular column
``cut'' from the original $C$, with which we can invoke 
the FMDV.
Our overall objective, is to jointly find: (1) an $m$-segmentation 
$(C_i : i \in [m])$
from all possible segmentation, denoted by $\mathbf{S}(C)$;
and  (2) furthermore find appropriate patterns 
$h_i \in \mathbf{H}(C_i)$ for each segment
$C_i$, such that the entire $C$ can be validated with a low
expected FPR. Also note that because we limit pattern enumeration
in offline-indexing to columns of at most $\tau$ tokens,
we would not find candidate patterns longer than $\tau$ in offline-index,
and can thus naturally limit the span of each segment to at most $\tau$
($e_i - s_i < \tau$, $\forall i$).
We can write this as an optimization problem FMDV-V defined as follows:
}


\small
\begin{align}
 \text{(FMDV-V)}~ \min_{\substack{ h_1 \dots h_m \\ h_i \in \mathbf{H}(C_i) \\ (C_i: i \in [m]) \in \mathbf{S}(C)}}~~~& \sum_{h_i} \text{FPR}_\mathbf{T}(h_i)   \label{eqn:fmdvv_obj} \\ 
 \mbox{s.t.} ~~
% & (h_1, h_2, \ldots, h_n) \in \mathbf{H}(C) \label{eqn:fmdvv_concat} \\
& \sum_{h_i} \text{FPR}_\mathbf{T}(h_i) \leq r \label{eqn:fmdvv_fpr} \\
 & \text{Cov}_\mathbf{T}(h_i) \geq m,~\forall h_i \label{eqn:fmdvv_cov}
\end{align}
\normalsize

In FMDV-V, we are optimizing over all possible segmentation
$(C_i : i \in [m]) \in \mathbf{S}(C)$, and for each $C_i$
all possible hypothesis patterns $h_i \in \mathbf{H}(C_i)$.
Our objective in Equation~\eqref{eqn:fmdvv_obj} is 
to minimize the sum of 
$\text{FPR}_\mathbf{T}(h_i)$ for all $h_i$.
We should note that this corresponds to a ``pessimistic'' 
approach that assumes non-conforming rows 
of each $h_i$ are disjoint at a row-level, thus needing to
to sum them up in the objective function.
(An alternative ``optimistic'' approach could assume
non-conforming values in different segments 
to overlap at a row-level, in which case
we can use \textit{max} in place of \textit{sum}.
We find this to be less effective and will omit details in the interest of space).

%The FPR and coverage requirements in Equation~\eqref{eqn:fmdvv_fpr}
%and~\eqref{eqn:fmdvv_cov} are similar to their counterparts in FMDV.


We can show that the minimum FRP scores of 
$m$-segmentation optimized in Equation~\eqref{eqn:fmdvv_obj} have 
\textit{optimal substructure}~\cite{cormen2009introduction}, which makes
it amenable to dynamic programming (without exhaustive
enumeration). Specifically, 
we can show that the following relationship holds:

\scriptsize
\begin{equation}
\vspace{-2mm}
\label{eqn:substructure}
\begin{split}
\text{minFRP}(C[s, e]) & = \\ \min \bigg(&  \min_{h \in \mathbf{P}(C[s, e])} \text{FPR}_{\mathbf{T}}(h), \\ 
&  \min_{t \in[s, e-1]}{\Big( \text{minFPR}(C[s, t]) + \text{minFPR}(C[t+1, e]) \Big)}\bigg)
\end{split}
\end{equation}
\normalsize

Here, minFRP$(C[s, e])$ is the minimum FRP score with
vertical splits as optimized in 
Equation~\eqref{eqn:fmdvv_obj}, for a sub-column
corresponding to the segment
$C[s, e]$ from token-position $s$ to $e$.
Note that $C[1, n]$ corresponds to the original query column $C$,
and minFRP$(C[1, n])$ is the score we want to optimize.
Equation~\eqref{eqn:substructure} shows how this
can be computed incrementally.
Specifically, minFRP$(C[s, e])$ is the minimum of:
(1) $\min_{h \in \mathbf{P}(C[s, e])}\text{FPR}_{\mathbf{T}}(h)$,
which is the FRP score 
of treating $C[s, e]$ as one column (with no splits), solvable
using FMDV;
and (2) $\min_{ t \in [s, e-1]}{\big( \text{minFPR}(C[s, t]) + \text{minFPR}(C[t+1, e]) \big)}$, which is the best minFRP scores from 
all possible two-way splits that
can be solved optimally in polynomial time using bottom-up 
dynamic-programming.


%revised
\iftoggle{fullversion}{
\begin{example}
\label{ex:fmdv-v}
Continue with Example~\ref{ex:align}.
The aligned sequence of column $C$ in Figure~\ref{fig:example-split}
has 29 tokens, corresponding to $C[1, 29]$. 
The sub-sequence $C[4, 14]$ maps to identical
values ``\val{02/18/2015 00:00:00}'' for all rows, 
which can be seen as a ``sub-column'' split from $C$.

Using Equation~\eqref{eqn:substructure}, 
\text{minFRP}$(C[4, 14])$ of this sub-column 
can be computed as 
the minimum of:
(1) Not splitting of $C[4, 14]$, or
$\min_{h \in \mathbf{P}(C[4, 14])}\text{FPR}_{\mathbf{T}}(h)$,
computed using FMDV; and
(2) Further splitting $C[4, 14]$ into two, 
where the best score is
$\min_{t \in[4, 13]}{\Big( \text{minFPR}(C[4, t]) + \text{minFPR}(C[t+1, 14]) \Big)}$, which can in turn be recursively computed.
Suppose we compute (1) to have FPR of 0.004\%, 
and the best of (2) to have FPR of 0.01\% (say, splitting 
into ``\val{02/18/2015}'' and ``\val{00:00:00}'').
Overall, not splitting $C[4, 14]$ is the best option.

Each such $C[s, e]$ can be computed bottom-up, until reaching
the top-level. %Specifically, the top-level
%\text{minFRP}(C[1, 29]) can be computed as 
%the minimum of:
%(1) Not splitting $C[1, 29]$: 
%or $\min_{h \in \mathbf{P}(C[1, 29])}\text{FPR}_{\mathbf{T}}(h)$
% computed from FMDV. 
%Because $C[1, 29]$ is sparsely represented in $\mathbf{T}$,
%in FMDV we could not find feasible solutions 
%meeting the coverage requirement. And
%(2) Splitting $C[1, 29]$: we find splitting along
%$C[1, 14]$ and $C[15, 29]$ to have the minimum FPR
%(which are in turn recursively split). 
The resulting split
minimizes the overall FPR and is solution to FMDV-V.
\end{example}
}%iftoggle

\revised{
We would like to highlight that by using vertical-cuts, we can safely
ignore wide columns with more than $\tau$ tokens during offline
indexing (Section~\ref{sec:architecture}), without
affecting result quality. As a concrete example, 
when we encounter a column like
in Figure~\ref{fig:example-split}, brute-force enumeration would
generate at least $4^{29}$ patterns, which is impractically large
and why it is omitted given a smaller token-length limit $\tau$ (e.g., 13) 
in offline indexing. However, when we encounter 
this column Figure~\ref{fig:example-split}
as a query column, we can still generate valid domain patterns
with the help of vertical-cuts,
%revised
\iftoggle{fullversion}
{
as we have seen in 
Example~\ref{ex:fmdv-v},
} as long as each segment has at most
$\tau$ tokens. This key benefit of vertical-cuts 
greatly speeds up offline-indexing without compromising result quality.
}









==> auto-validate.bib.2 <==
% Encoding: windows-1252

@ARTICLE{abedjan2016,
  author = {Abedjan, Ziawasch and Chu, Xu and Deng, Dong and Fernandez, Raul
	Castro and Ilyas, Ihab F and Ouzzani, Mourad and Papotti, Paolo and
	Stonebraker, Michael and Tang, Nan},
  title = {Detecting Data Errors: Where are we and what needs to be done?},
  journal = {VLDB},
  year = {2016},
  volume = {9},
  number = {12},
  publisher = {VLDB Endowment}
}

@inproceedings{bogatu2020dataset,
  title={Dataset Discovery in Data Lakes},
  author={Bogatu, Alex and Fernandes, Alvaro AA and Paton, Norman W and Konstantinou, Nikolaos},
  booktitle={2020 IEEE 36th International Conference on Data Engineering (ICDE)},
  pages={709--720},
  year={2020},
  organization={IEEE}
}

@article{qahtan13pattern,
  title={Pattern Functional Dependencies for Data Cleaning},
  author={Qahtan, Abdulhakim and Tang, Nan and Ouzzani, Mourad and Cao, Yang and Stonebraker, Michael},
  journal={Proceedings of the VLDB Endowment},
  volume={13},
  number={5}
}

@article{padhi2018flashprofile,
  title={FlashProfile: a framework for synthesizing data profiles},
  author={Padhi, Saswat and Jain, Prateek and Perelman, Daniel and Polozov, Oleksandr and Gulwani, Sumit and Millstein, Todd},
  journal={Proceedings of the ACM on Programming Languages},
  volume={2},
  number={OOPSLA},
  pages={1--28},
  year={2018},
  publisher={ACM New York, NY, USA}
}



@inproceedings{qahtan2018fahes,
  title={FAHES: A robust disguised missing values detector},
  author={Qahtan, Abdulhakim A and Elmagarmid, Ahmed and Castro Fernandez, Raul and Ouzzani, Mourad and Tang, Nan},
  booktitle={Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={2100--2109},
  year={2018}
}


@INPROCEEDINGS{abedjan2016dataxformer,
  author = {Abedjan, Ziawasch and Morcos, John and Ilyas, Ihab F and Ouzzani,
	Mourad and Papotti, Paolo and Stonebraker, Michael},
  title = {DataXFormer: A robust transformation discovery system},
  booktitle = {2016 IEEE 32nd International Conference on Data Engineering (ICDE)},
  year = {2016},
  pages = {1134--1145},
  organization = {IEEE}
}

@INPROCEEDINGS{abreu2014smelling,
  author = {Abreu, Rui and Cunha, J{\'a}come and Fernandes, Jo{\~a}o Paulo and
	Martins, Pedro and Perez, Alexandre and Saraiva, Jo{\~a}o},
  title = {Smelling faults in spreadsheets},
  booktitle = {Software Maintenance and Evolution (ICSME), 2014 IEEE International
	Conference on},
  year = {2014},
  organization = {IEEE}
}

@INPROCEEDINGS{afrati2009repair,
  author = {Afrati, Foto N and Kolaitis, Phokion G},
  title = {Repair checking in inconsistent databases: algorithms and complexity},
  booktitle = {Proceedings of the 12th International Conference on Database Theory},
  year = {2009},
  organization = {ACM}
}

@INPROCEEDINGS{arning1996linear,
  author = {Arning, Andreas and Agrawal, Rakesh and Raghavan, Prabhakar},
  title = {A Linear Method for Deviation Detection in Large Databases.},
  booktitle = {KDD},
  year = {1996}
}

@ARTICLE{arulselvan2014note,
  author = {Arulselvan, Ashwin},
  title = {A note on the set union knapsack problem},
  journal = {Discrete Applied Mathematics},
  year = {2014},
  volume = {169},
  publisher = {Elsevier}
}

@ARTICLE{asahiro2002complexity,
  author = {Asahiro, Yuichi and Hassin, Refael and Iwama, Kazuo},
  title = {Complexity of finding dense subgraphs},
  journal = {Discrete Applied Mathematics},
  year = {2002},
  volume = {121},
  pages = {15--26},
  number = {1-3},
  publisher = {Elsevier}
}

@ARTICLE{barron1998,
  author = {Barron, Andrew and Rissanen, Jorma and Yu, Bin},
  title = {The minimum description length principle in coding and modeling},
  journal = {IEEE Transactions on Information Theory},
  year = {1998},
  volume = {44},
  number = {6},
  publisher = {IEEE}
}

@INCOLLECTION{ben2005outlier,
  author = {Ben-Gal, Irad},
  title = {Outlier detection},
  booktitle = {Data mining and knowledge discovery handbook},
  publisher = {Springer},
  year = {2005}
}

@ARTICLE{bengio2003neural,
  author = {Bengio, Yoshua and Ducharme, R{\'e}jean and Vincent, Pascal and Jauvin,
	Christian},
  title = {A neural probabilistic language model},
  journal = {Journal of machine learning research},
  year = {2003},
  volume = {3},
  pages = {1137--1155},
  number = {Feb}
}

@ARTICLE{benjamini1995controlling,
  author = {Benjamini, Yoav and Hochberg, Yosef},
  title = {Controlling the false discovery rate: a practical and powerful approach
	to multiple testing},
  journal = {Journal of the Royal statistical society: series B (Methodological)},
  year = {1995}
}

@ARTICLE{berti2018discovery,
  author = {Berti-Equille, Laure and Harmouch, Hazar and Naumann, Felix and Novelli,
	No{\"e}l and Thirumuruganathan, Saravanan},
  title = {Discovery of genuine functional dependencies from relational data
	with missing values},
  journal = {VLDB},
  year = {2018}
}

@INPROCEEDINGS{bex2006,
  author = {Bex, Geert Jan and Neven, Frank and Schwentick, Thomas and Tuyls,
	Karl},
  title = {Inference of concise DTDs from XML data},
  booktitle = {VLDB},
  year = {2006}
}

@BOOK{biemann2011structure,
  title = {Structure discovery in natural language},
  publisher = {Springer Science \& Business Media},
  year = {2011},
  author = {Biemann, Chris and van den Bosch, Antal}
}

@INPROCEEDINGS{bohannon2005cost,
  author = {Bohannon, Philip and Fan, Wenfei and Flaster, Michael and Rastogi,
	Rajeev},
  title = {A cost-based model and effective heuristic for repairing constraints
	by value modification},
  booktitle = {Proceedings of the 2005 ACM SIGMOD international conference on Management
	of data},
  year = {2005},
  pages = {143--154},
  organization = {ACM}
}

@INPROCEEDINGS{bohannon2007,
  author = {Bohannon, Philip and Fan, Wenfei and Geerts, Floris and Jia, Xibei
	and Kementsietsidis, Anastasios},
  title = {Conditional functional dependencies for data cleaning},
  booktitle = {ICDE},
  year = {2007},
  organization = {IEEE}
}

@INPROCEEDINGS{breck2019data,
  author = {Breck, Eric and Polyzotis, Neoklis and Roy, Sudip and Whang, Steven
	and Zinkevich, Martin},
  title = {Data Validation for Machine Learning},
  booktitle = {Conference on Systems and Machine Learning (SysML). https://www.
	sysml. cc/doc/2019/167. pdf},
  year = {2019}
}

@ARTICLE{brewer2012cap,
  author = {Brewer, Eric},
  title = {CAP Twelve years Later: how the},
  journal = {Computer},
  year = {2012},
  number = {2},
  publisher = {IEEE}
}

@ARTICLE{bruglieri2004cardinality,
  author = {Bruglieri, Maurizio and Maffioli, Francesco and Ehrgott, Matthias},
  title = {Cardinality constrained minimum cut problems: complexity and algorithms},
  journal = {Discrete Applied Mathematics},
  year = {2004},
  volume = {137},
  pages = {311--341},
  number = {3},
  publisher = {Elsevier}
}

@ARTICLE{cafarella2008,
  author = {Cafarella, Michael J and Halevy, Alon and Wang, Daisy Zhe and Wu,
	Eugene and Zhang, Yang},
  title = {Webtables: exploring the power of tables on the web},
  journal = {VLDB},
  year = {2008},
  volume = {1},
  number = {1},
  publisher = {VLDB Endowment}
}

@ARTICLE{casellar,
  author = {Casella, George and Berger, Roger},
  title = {R. 2001, Statistical Inference},
  journal = {Duxbury Press}
}

@BOOK{casella2002statistical,
  title = {Statistical inference},
  publisher = {Duxbury Pacific Grove, CA},
  year = {2002},
  author = {Casella, George and Berger, Roger L},
  volume = {2}
}

@ARTICLE{webtables,
  author = {Chakrabarti, Kaushik and Chaudhuri, Surajit and Chen, Zhimin and
	Ganjam, Kris and He, Yeye and Redmond, WA},
  title = {Data services leveraging Bing's data assets.},
  journal = {IEEE Data Eng. Bull.},
  year = {2016},
  volume = {39},
  number = {3}
}

@ARTICLE{chandola2009anomaly,
  author = {Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  title = {Anomaly detection: A survey},
  journal = {ACM computing surveys (CSUR)},
  year = {2009},
  volume = {41},
  number = {3},
  publisher = {ACM}
}

@ARTICLE{chandola2007,
  author = {Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  title = {Outlier detection: A survey},
  journal = {ACM Computing Surveys},
  year = {2007}
}

@INPROCEEDINGS{chen1996empirical,
  author = {Chen, Stanley F and Goodman, Joshua},
  title = {An empirical study of smoothing techniques for language modeling},
  booktitle = {Proceedings of the 34th annual meeting on Association for Computational
	Linguistics},
  year = {1996},
  organization = {ACL}
}

@ARTICLE{chen2014fast,
  author = {Chen, Zhimin and Narasayya, Vivek and Chaudhuri, Surajit},
  title = {Fast foreign-key detection in Microsoft SQL server PowerPivot for
	Excel},
  journal = {Proceedings of the VLDB Endowment},
  year = {2014},
  volume = {7},
  pages = {1417--1428},
  number = {13},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{cheung2016,
  author = {Cheung, Shing-Chi and Chen, Wanjun and Liu, Yepang and Xu, Chang},
  title = {CUSTODES: automatic spreadsheet cell clustering and smell detection
	using strong and weak features},
  booktitle = {Proceedings of the 38th International Conference on Software Engineering},
  year = {2016}
}

@ARTICLE{Chiang2008,
  author = {Chiang, Fei and Miller, Ren{\'e}e J},
  title = {Discovering data quality rules},
  journal = {Proceedings of the VLDB Endowment},
  year = {2008},
  volume = {1},
  pages = {1166--1177},
  number = {1},
  publisher = {VLDB Endowment}
}

@ARTICLE{chiang2008discovering,
  author = {Chiang, Fei and Miller, Ren{\'e}e J},
  title = {Discovering data quality rules},
  journal = {VLDB},
  year = {2008},
  volume = {1},
  number = {1},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{chu2015tegra,
  author = {Chu, Xu and He, Yeye and Chakrabarti, Kaushik and Ganjam, Kris},
  title = {Tegra: Table extraction by global record alignment},
  booktitle = {SIGMOD},
  year = {2015}
}

@ARTICLE{chu2013,
  author = {Chu, Xu and Ilyas, Ihab F and Papotti, Paolo},
  title = {Discovering denial constraints},
  journal = {VLDB},
  year = {2013},
  volume = {6},
  number = {13},
  publisher = {VLDB Endowment}
}

@ARTICLE{chu2013discovering,
  author = {Chu, Xu and Ilyas, Ihab F and Papotti, Paolo},
  title = {Discovering denial constraints},
  journal = {VLDB},
  year = {2013},
  volume = {6},
  number = {13},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{chu2013holistic,
  author = {Chu, Xu and Ilyas, Ihab F and Papotti, Paolo},
  title = {Holistic data cleaning: Putting violations into context},
  booktitle = {ICDE},
  year = {2013},
  organization = {IEEE}
}

@INPROCEEDINGS{chu2015,
  author = {Chu, Xu and Morcos, John and Ilyas, Ihab F and Ouzzani, Mourad and
	Papotti, Paolo and Tang, Nan and Ye, Yin},
  title = {Katara: A data cleaning system powered by knowledge bases and crowdsourcing},
  booktitle = {SIGMOD},
  year = {2015}
}

@ARTICLE{church1990word,
  author = {Church, Kenneth Ward and Hanks, Patrick},
  title = {Word association norms, mutual information, and lexicography},
  journal = {Computational linguistics},
  year = {1990},
  volume = {16},
  number = {1},
  publisher = {MIT Press}
}

@ARTICLE{clauset2009power,
  author = {Clauset, Aaron and Shalizi, Cosma Rohilla and Newman, Mark EJ},
  title = {Power-law distributions in empirical data},
  journal = {SIAM review},
  year = {2009},
  volume = {51},
  number = {4},
  publisher = {SIAM}
}

@INPROCEEDINGS{collobert2008unified,
  author = {Collobert, Ronan and Weston, Jason},
  title = {A unified architecture for natural language processing: Deep neural
	networks with multitask learning},
  booktitle = {Proceedings of the 25th international conference on Machine learning},
  year = {2008},
  pages = {160--167},
  organization = {ACM}
}

@INPROCEEDINGS{cong2007,
  author = {Cong, Gao and Fan, Wenfei and Geerts, Floris and Jia, Xibei and Ma,
	Shuai},
  title = {Improving data quality: Consistency and accuracy},
  booktitle = {VLDB},
  year = {2007}
}

@INPROCEEDINGS{cong2007improving,
  author = {Cong, Gao and Fan, Wenfei and Geerts, Floris and Jia, Xibei and Ma,
	Shuai},
  title = {Improving data quality: Consistency and accuracy},
  booktitle = {Proceedings of the 33rd international conference on Very large data
	bases},
  year = {2007},
  pages = {315--326},
  organization = {VLDB Endowment}
}

@ARTICLE{cormode2005improved,
  author = {Cormode, Graham and Muthukrishnan, Shan},
  title = {An improved data stream summary: the count-min sketch and its applications},
  journal = {Journal of Algorithms},
  year = {2005},
  volume = {55},
  number = {1},
  publisher = {Elsevier}
}

@INPROCEEDINGS{cormode2005summarizing,
  author = {Cormode, Graham and Muthukrishnan, S},
  title = {Summarizing and mining skewed data streams},
  booktitle = {Proceedings of the 2005 SIAM International Conference on Data Mining},
  year = {2005},
  organization = {SIAM}
}

@INPROCEEDINGS{dasu2002mining,
  author = {Dasu, Tamraparni and Johnson, Theodore and Muthukrishnan, Shanmugauelayut
	and Shkapenyuk, Vladislav},
  title = {Mining database structure; or, how to build a data quality browser},
  booktitle = {SIGMOD},
  year = {2002}
}

@INPROCEEDINGS{dayal2009data,
  author = {Dayal, Umeshwar and Castellanos, Malu and Simitsis, Alkis and Wilkinson,
	Kevin},
  title = {Data integration flows for business intelligence},
  booktitle = {Proceedings of the 12th International Conference on Extending Database
	Technology: Advances in Database Technology},
  year = {2009},
  pages = {1--11}
}

@INPROCEEDINGS{deng2017data,
  author = {Deng, Dong and Fernandez, Raul Castro and Abedjan, Ziawasch and Wang,
	Sibo and Stonebraker, Michael and Elmagarmid, Ahmed K and Ilyas,
	Ihab F and Madden, Samuel and Ouzzani, Mourad and Tang, Nan},
  title = {The Data Civilizer System.},
  booktitle = {Cidr},
  year = {2017}
}

@Misc{Enterprise2016,
  author = {Enterprise, Trifacta Wrangler},
  title  = {Trifacta wrangler (2015)},
  year   = {2016},
}

@INPROCEEDINGS{fan2014,
  author = {Fan, Grace and Fan, Wenfei and Geerts, Floris},
  title = {Detecting errors in numeric attributes},
  booktitle = {International Conference on Web-Age Information Management},
  year = {2014},
  organization = {Springer}
}

@ARTICLE{fan2009reasoning,
  author = {Fan, Wenfei and Jia, Xibei and Li, Jianzhong and Ma, Shuai},
  title = {Reasoning about record matching rules},
  journal = {VLDB},
  year = {2009},
  volume = {2},
  number = {1},
  publisher = {VLDB Endowment}
}

@ARTICLE{fisher2005pads,
  author = {Fisher, Kathleen and Gruber, Robert},
  title = {PADS: a domain-specific language for processing ad hoc data},
  journal = {ACM Sigplan Notices},
  year = {2005},
  volume = {40},
  pages = {295--304},
  number = {6},
  publisher = {ACM New York, NY, USA}
}

@ARTICLE{fisher2008dirt,
  author = {Fisher, Kathleen and Walker, David and Zhu, Kenny Q and White, Peter},
  title = {From dirt to shovels: fully automatic tool generation from ad hoc
	data},
  journal = {ACM SIGPLAN Notices},
  year = {2008},
  volume = {43},
  pages = {421--434},
  number = {1},
  publisher = {ACM New York, NY, USA}
}

@ARTICLE{freeman1996make,
  author = {Freeman, David},
  title = {How to make spreadsheets error-proof},
  journal = {Journal of Accountancy},
  year = {1996},
  volume = {181},
  number = {5},
  publisher = {American Institute of Certified Public Accountants}
}

@INPROCEEDINGS{ganjisaffar2011qspell,
  author = {Ganjisaffar, Yasser and Zilio, Andrea and Javanmardi, Sara and Cetindil,
	Inci and Sikka, Manik and Katumalla, Sandeep and Khatib, Narges and
	Li, Chen and Lopes, Cristina},
  title = {qspell: Spelling correction of web search queries using ranking models
	and iterative correction},
  booktitle = {Spelling Alteration for Web Search Workshop},
  year = {2011}
}

@ARTICLE{geerts2013llunatic,
  author = {Geerts, Floris and Mecca, Giansalvatore and Papotti, Paolo and Santoro,
	Donatello},
  title = {The LLUNATIC data-cleaning framework},
  journal = {Proceedings of the VLDB Endowment},
  year = {2013},
  volume = {6},
  pages = {625--636},
  number = {9},
  publisher = {VLDB Endowment}
}

@BOOK{gennick2010sql,
  title = {SQL Pocket Guide: A Guide to SQL Usage},
  publisher = {" O'Reilly Media, Inc."},
  year = {2010},
  author = {Gennick, Jonathan}
}

@ARTICLE{go2009twitter,
  author = {Go, Alec and Bhayani, Richa and Huang, Lei},
  title = {Twitter sentiment classification using distant supervision},
  journal = {CS224N Project Report, Stanford},
  year = {2009},
  volume = {1},
  number = {2009}
}

@ARTICLE{golab2010data,
  author = {Golab, Lukasz and Karloff, Howard and Korn, Flip and Srivastava,
	Divesh},
  title = {Data auditor: Exploring data quality and semantics using pattern
	tableaux},
  journal = {VLDB},
  year = {2010},
  volume = {3},
  number = {1-2},
  publisher = {VLDB Endowment}
}

@ARTICLE{goldschmidt1994polynomial,
  author = {Goldschmidt, Olivier and Hochbaum, Dorit S},
  title = {A polynomial algorithm for the k-cut problem for fixed k},
  journal = {Mathematics of operations research},
  year = {1994},
  volume = {19},
  pages = {24--37},
  number = {1},
  publisher = {INFORMS}
}

@ARTICLE{gulwani2012,
  author = {Gulwani, Sumit and Harris, William R and Singh, Rishabh},
  title = {Spreadsheet data manipulation using examples},
  journal = {Communications of the ACM},
  year = {2012},
  volume = {55},
  number = {8},
  publisher = {ACM}
}

@ARTICLE{gupta2014outlier,
  author = {Gupta, Manish and Gao, Jing and Aggarwal, Charu C and Han, Jiawei},
  title = {Outlier detection for temporal data: A survey},
  journal = {TKDE},
  year = {2014},
  volume = {26},
  number = {9},
  publisher = {IEEE}
}

@INPROCEEDINGS{halevy2016goods,
  author = {Halevy, Alon and Korn, Flip and Noy, Natalya F and Olston, Christopher
	and Polyzotis, Neoklis and Roy, Sudip and Whang, Steven Euijong},
  title = {Goods: Organizing google's datasets},
  booktitle = {SIGMOD},
  year = {2016}
}

@ARTICLE{hall1992smoothed,
  author = {Hall, Peter and Marron, JS and Park, Byeong U},
  title = {Smoothed cross-validation},
  journal = {Probability theory and related fields},
  year = {1992},
  volume = {92},
  number = {1},
  publisher = {Springer}
}

@INPROCEEDINGS{harris2011spreadsheet,
  author = {Harris, William R and Gulwani, Sumit},
  title = {Spreadsheet table transformations from examples},
  booktitle = {ACM SIGPLAN Notices},
  year = {2011},
  volume = {46},
  number = {6},
  organization = {ACM}
}

@INPROCEEDINGS{he2016interactive,
  author = {He, Jian and Veltri, Enzo and Santoro, Donatello and Li, Guoliang
	and Mecca, Giansalvatore and Papotti, Paolo and Tang, Nan},
  title = {Interactive and deterministic data cleaning},
  booktitle = {SIGMOD},
  year = {2016}
}

@ARTICLE{he2018transform,
  author = {He, Yeye and Chu, Xu and Ganjam, Kris and Zheng, Yudian and Narasayya,
	Vivek and Chaudhuri, Surajit},
  title = {{Transform-data-by-example (TDE): an extensible search engine for
	data transformations}},
  journal = {VLDB},
  year = {2018},
  volume = {11},
  number = {10},
  publisher = {VLDB Endowment}
}

@ARTICLE{he2015,
  author = {He, Yeye and Ganjam, Kris and Chu, Xu},
  title = {{SEMA-JOIN: joining semantically-related tables using big table corpora}},
  journal = {VLDB},
  year = {2015},
  volume = {8},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{he2015sema,
  author = {He, Yeye and Ganjam, Kris and Chu, Xu},
  title = {{SEMA-JOIN: joining semantically-related tables using big table corpora}},
  journal = {VLDB},
  year = {2015},
  volume = {8},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{he2005,
  author = {He, Zengyou and Deng, Shengchun and Xu, Xiaofei},
  title = {An optimization model for outlier detection in categorical data},
  journal = {Advances in Intelligent Computing},
  year = {2005}
}

@INPROCEEDINGS{he2005optimization,
  author = {He, Zengyou and Deng, Shengchun and Xu, Xiaofei},
  title = {An optimization model for outlier detection in categorical data},
  booktitle = {International Conference on Intelligent Computing},
  year = {2005}
}

@INPROCEEDINGS{heer2015predictive,
  author = {Heer, Jeffrey and Hellerstein, Joseph M and Kandel, Sean},
  title = {Predictive Interaction for Data Transformation.},
  booktitle = {CIDR},
  year = {2015}
}

@ARTICLE{hellerstein2008,
  author = {Hellerstein, Joseph M},
  title = {Quantitative data cleaning for large databases},
  journal = {United Nations Economic Commission for Europe (UNECE)},
  year = {2008}
}

@INPROCEEDINGS{hochbaum,
  author = {Hochbaum, Dorit S},
  title = {Approximating covering and packing problems: set cover, vertex cover,
	independent set, and related problems},
  booktitle = {Approximation algorithms for NP-hard problems},
  year = {1996},
  organization = {PWS Publishing Co.}
}

@INPROCEEDINGS{hochbaum1996approximating,
  author = {Hochbaum, Dorit S},
  title = {Approximating covering and packing problems: set cover, vertex cover,
	independent set, and related problems},
  booktitle = {Approximation algorithms for NP-hard problems},
  year = {1996},
  organization = {PWS Publishing Co.}
}

@ARTICLE{hodge2004survey,
  author = {Hodge, Victoria and Austin, Jim},
  title = {A survey of outlier detection methodologies},
  journal = {Artificial intelligence review},
  year = {2004}
}

@INPROCEEDINGS{huang2018auto,
  author = {Huang, Zhipeng and He, Yeye},
  title = {{Auto-Detect: Data-Driven Error Detection in Tables}},
  booktitle = {SIGMOD},
  year = {2018}
}

@ARTICLE{huhtala1999tane,
  author = {Huhtala, Yka and K{\"a}rkk{\"a}inen, Juha and Porkka, Pasi and Toivonen,
	Hannu},
  title = {TANE: An efficient algorithm for discovering functional and approximate
	dependencies},
  journal = {The computer journal},
  year = {1999},
  volume = {42},
  number = {2},
  publisher = {OUP}
}

@BOOK{Ben-Gal05,
  title = {Data Mining and Knowledge Discovery Handbook: A Complete Guide for
	Practitioners and Researchers},
  publisher = {Kluwer Academic Publishers},
  year = {2005},
  author = {Ben-Gal I.},
  owner = {yeyehe},
  timestamp = {2018.10.02}
}

@INPROCEEDINGS{ilyas2018extracting,
  author = {Ilyas, Andrew and da Trindade, Joana MF and Fernandez, Raul Castro
	and Madden, Samuel},
  title = {Extracting syntactical patterns from databases},
  booktitle = {2018 IEEE 34th International Conference on Data Engineering (ICDE)},
  year = {2018},
  pages = {41--52},
  organization = {IEEE}
}

@INPROCEEDINGS{ilyas2004,
  author = {Ilyas, Ihab F and Markl, Volker and Haas, Peter and Brown, Paul and
	Aboulnaga, Ashraf},
  title = {CORDS: automatic discovery of correlations and soft functional dependencies},
  booktitle = {SIGMOD},
  year = {2004}
}

@INPROCEEDINGS{ilyas2004cords,
  author = {Ilyas, Ihab F and Markl, Volker and Haas, Peter and Brown, Paul and
	Aboulnaga, Ashraf},
  title = {CORDS: automatic discovery of correlations and soft functional dependencies},
  booktitle = {SIGMOD},
  year = {2004}
}

@INPROCEEDINGS{jin2017foofah,
  author = {Jin, Zhongjun and Anderson, Michael R and Cafarella, Michael and
	Jagadish, HV},
  title = {Foofah: Transforming data by example},
  booktitle = {Proceedings of the 2017 ACM International Conference on Management
	of Data},
  year = {2017},
  pages = {683--698},
  organization = {ACM}
}

@INPROCEEDINGS{kandel2011wrangler,
  author = {Kandel, Sean and Paepcke, Andreas and Hellerstein, Joseph and Heer,
	Jeffrey},
  title = {Wrangler: Interactive visual specification of data transformation
	scripts},
  booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing
	Systems},
  year = {2011},
  pages = {3363--3372},
  organization = {ACM}
}

@ARTICLE{kazai2013analysis,
  author = {Kazai, Gabriella and Kamps, Jaap and Milic-Frayling, Natasa},
  title = {An analysis of human factors and label accuracy in crowdsourcing
	relevance judgments},
  journal = {Information retrieval},
  year = {2013},
  volume = {16},
  number = {2},
  publisher = {Springer}
}

@INPROCEEDINGS{keogh2004towards,
  author = {Keogh, Eamonn and Lonardi, Stefano and Ratanamahatana, Chotirat Ann},
  title = {Towards parameter-free data mining},
  booktitle = {SIGKDD},
  year = {2004}
}

@ARTICLE{khuller1999budgeted,
  author = {Khuller, Samir and Moss, Anna and Naor, Joseph Seffi},
  title = {The budgeted maximum coverage problem},
  journal = {Information Processing Letters},
  year = {1999},
  volume = {70},
  number = {1},
  publisher = {Elsevier}
}

@ARTICLE{kivinen1995approximate,
  author = {Kivinen, Jyrki and Mannila, Heikki},
  title = {Approximate inference of functional dependencies from relations},
  journal = {Theoretical Computer Science},
  year = {1995},
  volume = {149},
  number = {1},
  publisher = {Elsevier}
}

@INPROCEEDINGS{knox1998algorithms,
  author = {Knox, Edwin M and Ng, Raymond T},
  title = {Algorithms for mining distance based outliers in large datasets},
  booktitle = {VLDB},
  year = {1998}
}

@TECHREPORT{BoostClean,
  author = {Sanjay Krishnan and Michael J. Franklin and Ken Goldberg and Eugene
	Wu},
  title = {BoostClean: Automated Error Detection and Repair for Machine Learning},
  year = {2017},
  owner = {yeye},
  timestamp = {2018.02.15}
}

@ARTICLE{krishnan2016activeclean,
  author = {Krishnan, Sanjay and Wang, Jiannan and Wu, Eugene and Franklin, Michael
	J and Goldberg, Ken},
  title = {ActiveClean: interactive data cleaning for statistical modeling},
  journal = {VLDB},
  year = {2016},
  volume = {9},
  number = {12},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{imagenet,
  author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  title = {Imagenet classification with deep convolutional neural networks},
  booktitle = {Advances in neural information processing systems},
  year = {2012}
}

@INPROCEEDINGS{Le2014,
  author = {Le, Vu and Gulwani, Sumit},
  title = {FlashExtract: a framework for data extraction by examples},
  booktitle = {ACM SIGPLAN Notices},
  year = {2014},
  volume = {49},
  number = {6},
  pages = {542--553},
  organization = {ACM}
}

@INPROCEEDINGS{le2014flashextract,
  author = {Le, Vu and Gulwani, Sumit},
  title = {FlashExtract: a framework for data extraction by examples},
  booktitle = {ACM SIGPLAN Notices},
  year = {2014},
  volume = {49},
  number = {6},
  organization = {ACM}
}

@BOOK{lee1997bayesian,
  title = {Bayesian statistics},
  publisher = {Arnold Publication},
  year = {1997},
  author = {Lee, Peter M}
}

@BOOK{lehmann2006testing,
  title = {Testing statistical hypotheses},
  publisher = {Springer Science \& Business Media},
  year = {2006},
  author = {Lehmann, Erich L and Romano, Joseph P}
}

@ARTICLE{leys2013detecting,
  author = {Leys, Christophe and Ley, Christophe and Klein, Olivier and Bernard,
	Philippe and Licata, Laurent},
  title = {Detecting outliers: Do not use standard deviation around the mean,
	use absolute deviation around the median},
  journal = {Journal of Experimental Social Psychology},
  year = {2013},
  volume = {49},
  number = {4},
  publisher = {Elsevier}
}

@INPROCEEDINGS{li2006exploring,
  author = {Li, Mu and Zhang, Yang and Zhu, Muhua and Zhou, Ming},
  title = {Exploring distributional similarity based models for query spelling
	correction},
  booktitle = {Proceedings of the 21st International Conference on Computational
	Linguistics and the 44th annual meeting of the Association for Computational
	Linguistics},
  year = {2006},
  organization = {ACL}
}

@INPROCEEDINGS{li2008regular,
  author = {Li, Yunyao and Krishnamurthy, Rajasekar and Raghavan, Sriram and
	Vaithyanathan, Shivakumar and Jagadish, HV},
  title = {Regular expression learning for information extraction},
  booktitle = {Proceedings of the Conference on Empirical Methods in Natural Language
	Processing},
  year = {2008},
  organization = {ACL}
}

@BOOK{lieberman2001your,
  title = {Your wish is my command: Programming by example},
  publisher = {Morgan Kaufmann},
  year = {2001},
  author = {Lieberman, Henry}
}

@ARTICLE{Forrester,
  author = {Cinny Little},
  title = {The Forrester Wave: Data Preparation Solutions, Q4 2018},
  owner = {yeyehe},
  timestamp = {2019.02.14}
}

@ARTICLE{liu2009learning,
  author = {Liu, Tie-Yan and others},
  title = {Learning to rank for information retrieval},
  journal = {Foundations and Trends{\textregistered} in Information Retrieval},
  year = {2009},
  volume = {3},
  pages = {225--331},
  number = {3},
  publisher = {Now Publishers, Inc.}
}

@ARTICLE{lopes2002,
  author = {Lopes, St{\'e}phane and Petit, Jean-Marc and Lakhal, Lotfi},
  title = {Functional and approximate dependency mining: database and FCA points
	of view},
  journal = {Journal of Experimental \& Theoretical Artificial Intelligence},
  year = {2002}
}

@INPROCEEDINGS{luec2011data,
  author = {Luec, Gord},
  title = {A data-driven approach for correcting search quaries},
  booktitle = {Spelling Alteration for Web Search Workshop},
  year = {2011}
}

@ARTICLE{manning2008scoring,
  author = {Manning, Christopher D and Raghavan, Prabhakar and Sch{\"u}tze, Hinrich},
  title = {Scoring, term weighting and the vector space model},
  journal = {Introduction to information retrieval},
  year = {2008},
  volume = {100},
  publisher = {Cambridge University Press}
}

@BOOK{pooling,
  title = {Evaluation in information retrieval, Stanford NLP Group, \url{https://www.gartner.com/doc/3204817/forecast-snapshot-selfservice-data-preparaGroup}},
  publisher = {Cambridge University Press},
  author = {Christopher D. Manning and Prabhakar Raghavan and Hinrich Schutze},
  owner = {yeyehe},
  timestamp = {2019.02.14},
  url = {\url{https://www.gartner.com/doc/3204817/forecast-snapshot-selfservice-data-preparation}}
}

@ARTICLE{mariet2016outlier,
  author = {Mariet, Zelda and Harding, Rachael and Madden, Sam and others},
  title = {Outlier Detection in Heterogeneous Datasets using Automatic Tuple
	Expansion},
  journal = {MIT Technical Report},
  year = {2016}
}

@ARTICLE{Ziemann16,
  author = {Mark Ziemann, Yotam Eren and Assam El-Osta},
  title = {Gene name errors are widespread in the scientific literature},
  journal = {Genome Biology},
  year = {2016},
  owner = {yeyehe},
  timestamp = {2018.10.01}
}

@ARTICLE{maronna1976robust,
  author = {Maronna, Ricardo Antonio},
  title = {Robust M-estimators of multivariate location and scatter},
  journal = {The annals of statistics},
  year = {1976},
  publisher = {JSTOR}
}

@BOOK{maronna2018robust,
  title = {Robust Statistics: Theory and Methods (with R)},
  publisher = {Wiley},
  year = {2018},
  author = {Maronna, Ricardo A and Martin, R Douglas and Yohai, Victor J and
	Salibi{\'a}n-Barrera, Mat{\'\i}as}
}

@INPROCEEDINGS{differential-privacy,
  author = {McSherry, Frank and Talwar, Kunal},
  title = {Mechanism design via differential privacy},
  booktitle = {Foundations of Computer Science, 2007. FOCS'07. 48th Annual IEEE
	Symposium on},
  year = {2007},
  organization = {IEEE}
}

@INPROCEEDINGS{mikolov2010recurrent,
  author = {Mikolov, Tom{\'a}{\v{s}} and Karafi{\'a}t, Martin and Burget, Luk{\'a}{\v{s}}
	and {\v{C}}ernock{\`y}, Jan and Khudanpur, Sanjeev},
  title = {Recurrent neural network based language model},
  booktitle = {Eleventh annual conference of the international speech communication
	association},
  year = {2010}
}

@INPROCEEDINGS{word2vec,
  author = {Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg
	S and Dean, Jeff},
  title = {Distributed representations of words and phrases and their compositionality},
  booktitle = {Advances in neural information processing systems},
  year = {2013}
}

@INPROCEEDINGS{mintz2009distant,
  author = {Mintz, Mike and Bills, Steven and Snow, Rion and Jurafsky, Dan},
  title = {Distant supervision for relation extraction without labeled data},
  booktitle = {Proceedings of the Joint Conference of the 47th Annual Meeting of
	the ACL and the 4th International Joint Conference on Natural Language
	Processing of the AFNLP: Volume 2-Volume 2},
  year = {2009},
  organization = {ACL}
}

@BOOK{neter1996applied,
  title = {Applied linear statistical models},
  publisher = {Irwin Chicago},
  year = {1996},
  author = {Neter, John and Kutner, Michael H and Nachtsheim, Christopher J and
	Wasserman, William},
  volume = {4}
}

@ARTICLE{Neyman33,
  author = {Neyman, J. and Pearson, E. S.},
  title = {On the problem of the most efficient tests of statistical hypotheses},
  journal = {Phil. Trans. R. Soc. Lond. A.},
  year = {1933}
}

@ARTICLE{padhi2017flashprofile,
  author = {Padhi, Saswat and Jain, Prateek and Perelman, Daniel and Polozov,
	Oleksandr and Gulwani, Sumit and Millstein, Todd D},
  title = {FlashProfile: Interactive Synthesis of Syntactic Profiles.},
  year = {2017}
}

@INPROCEEDINGS{pande2017effective,
  author = {Pande, Harshit},
  title = {Effective search space reduction for spell correction using character
	neural embeddings},
  booktitle = {Proceedings of the 15th Conference of the European Chapter of the
	ACL: Volume 2, Short Papers},
  year = {2017},
  volume = {2}
}

@INPROCEEDINGS{panko2008,
  author = {Panko, Raymond R},
  title = {Spreadsheet errors: What we know. what we think we can do},
  year = {2008},
  journal = {Symposium on Risk of Spreadsheets}
}

@ARTICLE{panko1998,
  author = {Panko, Raymond R},
  title = {What we know about spreadsheet errors},
  journal = {Journal of Organizational and End User Computing (JOEUC)},
  year = {1998}
}

@ARTICLE{papenbrock2015data,
  author = {Papenbrock, Thorsten and Bergmann, Tanja and Finke, Moritz and Zwiener,
	Jakob and Naumann, Felix},
  title = {Data profiling with metanome},
  journal = {VLDB},
  year = {2015},
  volume = {8},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{parzen1962estimation,
  author = {Parzen, Emanuel},
  title = {On estimation of a probability density function and mode},
  journal = {The annals of mathematical statistics},
  year = {1962},
  volume = {33},
  number = {3},
  publisher = {JSTOR}
}

@INPROCEEDINGS{patel2019big,
  author = {Patel, Hiren and Jindal, Alekh and Szyperski, Clemens},
  title = {Big Data Processing at Microsoft: Hyper Scale, Massive Complexity,
	and Minimal Cost},
  booktitle = {Proceedings of the ACM Symposium on Cloud Computing},
  year = {2019},
  pages = {490--490}
}

@INPROCEEDINGS{polyzotis2017data,
  author = {Polyzotis, Neoklis and Roy, Sudip and Whang, Steven Euijong and Zinkevich,
	Martin},
  title = {Data management challenges in production machine learning},
  booktitle = {Proceedings of the 2017 ACM International Conference on Management
	of Data},
  year = {2017},
  pages = {1723--1726}
}

@INPROCEEDINGS{powell2009,
  author = {Powell, Stephen G and Baker, Kenneth R and Lawson, Barry},
  title = {Errors in operational spreadsheets: A review of the state of the
	art},
  booktitle = {System Sciences, 2009. HICSS'09},
  year = {2009}
}

@INPROCEEDINGS{priedhorsky2007creating,
  author = {Priedhorsky, Reid and Chen, Jilin and Lam, Shyong Tony K and Panciera,
	Katherine and Terveen, Loren and Riedl, John},
  title = {Creating, destroying, and restoring value in Wikipedia},
  booktitle = {Proceedings of the 2007 international ACM conference on Supporting
	group work},
  year = {2007},
  organization = {ACM}
}

@INPROCEEDINGS{qahtan2018fahes,
  author = {Qahtan, Abdulhakim and Elmagarmid, Ahmed and Ouzzani, Mourad and
	Tang, Nan},
  title = {FAHES: Detecting disguised missing values},
  booktitle = {ICDE},
  year = {2018},
  organization = {IEEE}
}

@ARTICLE{rahman2018icarus,
  author = {Rahman, Protiva and Hebert, Courtney and Nandi, Arnab},
  title = {ICARUS: minimizing human effort in iterative data completion},
  journal = {VLDB},
  year = {2018},
  volume = {11},
  number = {13},
  publisher = {VLDB Endowment}
}

@ARTICLE{squad,
  author = {Rajpurkar, Pranav and Zhang, Jian and Lopyrev, Konstantin and Liang,
	Percy},
  title = {Squad: 100,000+ questions for machine comprehension of text},
  journal = {arXiv preprint arXiv:1606.05250},
  year = {2016}
}

@INPROCEEDINGS{raman2001potter,
  author = {Raman, Vijayshankar and Hellerstein, Joseph M},
  title = {Potter's wheel: An interactive data cleaning system},
  booktitle = {VLDB},
  year = {2001},
  volume = {1}
}

@ARTICLE{holoclean,
  author = {Rekatsinas, Theodoros and Chu, Xu and Ilyas, Ihab F and R{\'e}, Christopher},
  title = {Holoclean: Holistic data repairs with probabilistic inference},
  journal = {VLDB},
  year = {2017},
  volume = {10},
  number = {11},
  publisher = {VLDB Endowment}
}

@ARTICLE{rousseeuw1993alternatives,
  author = {Rousseeuw, Peter J and Croux, Christophe},
  title = {Alternatives to the median absolute deviation},
  journal = {Journal of the American Statistical association},
  year = {1993},
  volume = {88},
  number = {424},
  publisher = {Taylor \& Francis}
}

@BOOK{rozenberg2012handbook,
  title = {Handbook of Formal Languages: Volume 3 Beyond Words},
  publisher = {Springer Science \& Business Media},
  year = {2012},
  author = {Rozenberg, Grzegorz and Salomaa, Arto}
}

@BOOK{Schutze2008,
  title = {Introduction to information retrieval},
  publisher = {Cambridge University Press},
  year = {2008},
  author = {Sch{\"u}tze, Hinrich and Manning, Christopher D and Raghavan, Prabhakar},
  volume = {39}
}

@INPROCEEDINGS{schutze2008introduction,
  author = {Sch{\"u}tze, Hinrich and Manning, Christopher D and Raghavan, Prabhakar},
  title = {Introduction to information retrieval},
  booktitle = {Proceedings of the international communication of association for
	computing machinery conference},
  year = {2008},
  pages = {260}
}

@INPROCEEDINGS{schelter2019unit,
  author = {Schelter, Sebastian and Biessmann, Felix and Lange, Dustin and Rukat,
	Tammo and Schmidt, Phillipp and Seufert, Stephan and Brunelle, Pierre
	and Taptunov, Andrey},
  title = {Unit Testing Data with Deequ},
  booktitle = {Proceedings of the 2019 International Conference on Management of
	Data},
  year = {2019},
  pages = {1993--1996}
}

@INPROCEEDINGS{schelter2019differential,
  author = {Schelter, Sebastian and Grafberger, Stefan and Schmidt, Philipp and
	Rukat, Tammo and Kiessling, Mario and Taptunov, Andrey and Biessmann,
	Felix and Lange, Dustin},
  title = {Differential Data Quality Verification on Partitioned Data},
  booktitle = {2019 IEEE 35th International Conference on Data Engineering (ICDE)},
  year = {2019},
  pages = {1940--1945},
  organization = {IEEE}
}

@ARTICLE{schelter2018automating,
  author = {Schelter, Sebastian and Lange, Dustin and Schmidt, Philipp and Celikel,
	Meltem and Biessmann, Felix and Grafberger, Andreas},
  title = {Automating large-scale data quality verification},
  journal = {Proceedings of the VLDB Endowment},
  year = {2018},
  volume = {11},
  pages = {1781--1794},
  number = {12},
  publisher = {VLDB Endowment}
}

@ARTICLE{shachaf2010beyond,
  author = {Shachaf, Pnina and Hara, Noriko},
  title = {Beyond vandalism: Wikipedia trolls},
  journal = {Journal of Information Science},
  year = {2010},
  volume = {36},
  number = {3},
  publisher = {Sage Publications Sage UK: London, England}
}

@inproceedings{swami2020data,
  title={Data Sentinel: A Declarative Production-Scale Data Validation Platform},
  author={Swami, Arun and Vasudevan, Sriram and Huyn, Joojay},
  booktitle={2020 IEEE 36th International Conference on Data Engineering (ICDE)},
  pages={1579--1590},
  year={2020},
  organization={IEEE}
}


@ARTICLE{singh2016blinkfill,
  author = {Singh, Rishabh},
  title = {Blinkfill: Semi-supervised programming by example for syntactic string
	transformations},
  journal = {VLDB},
  year = {2016},
  volume = {9},
  number = {10},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{singh2016transforming,
  author = {Singh, Rishabh and Gulwani, Sumit},
  title = {Transforming spreadsheet data types using examples},
  booktitle = {Acm Sigplan Notices},
  year = {2016}
}

@ARTICLE{singhmelford,
  author = {Singh, Rishabh and Livshits, Benjamin and Zorn, Benjamin},
  title = {Melford: Using Neural Networks to Find Spreadsheet Errors},
  journal = {MSR technical report}
}

@ARTICLE{stoer1997simple,
  author = {Stoer, Mechthild and Wagner, Frank},
  title = {A simple min-cut algorithm},
  journal = {Journal of the ACM (JACM)},
  year = {1997},
  volume = {44},
  pages = {585--591},
  number = {4},
  publisher = {ACM}
}

@INPROCEEDINGS{surdeanu2010simple,
  author = {Surdeanu, Mihai and McClosky, David and Tibshirani, Julie and Bauer,
	John and Chang, Angel X and Spitkovsky, Valentin I and Manning, Christopher
	D},
  title = {A Simple Distant Supervision Approach for the TAC-KBP Slot Filling
	Task.},
  booktitle = {TAC},
  year = {2010}
}

@ARTICLE{tax2004support,
  author = {Tax, David MJ and Duin, Robert PW},
  title = {Support vector data description},
  journal = {Machine learning},
  year = {2004},
  volume = {54},
  number = {1},
  publisher = {Springer}
}

@BOOK{voorhees2005trec,
  title = {TREC: Experiment and evaluation in information retrieval},
  publisher = {MIT press Cambridge},
  year = {2005},
  author = {Voorhees, Ellen M and Harman, Donna K and others},
  volume = {1}
}

@INPROCEEDINGS{wang2017,
  author = {Wang, Yue and He, Yeye},
  title = {Synthesizing mapping relationships using table corpus},
  booktitle = {SIGMOD},
  year = {2017}
}

@INPROCEEDINGS{whitelaw2009using,
  author = {Whitelaw, Casey and Hutchinson, Ben and Chung, Grace Y and Ellis,
	Gerard},
  title = {Using the web for language independent spellchecking and autocorrection},
  booktitle = {Proceedings of the 2009 Conference on Empirical Methods in Natural
	Language Processing: Volume 2-Volume 2},
  year = {2009},
  organization = {ACL}
}

@ARTICLE{yaghmazadeh2018automated,
  author = {Yaghmazadeh, Navid and Wang, Xinyu and Dillig, Isil},
  title = {Automated migration of hierarchical data to relational tables using
	programming-by-example},
  journal = {Proceedings of the VLDB Endowment},
  year = {2018},
  volume = {11},
  pages = {580--593},
  number = {5},
  publisher = {VLDB Endowment}
}

@INPROCEEDINGS{yakout2013don,
  author = {Yakout, Mohamed and Berti-{\'E}quille, Laure and Elmagarmid, Ahmed
	K},
  title = {Don't be SCAREd: use SCalable Automatic REpairing with maximal likelihood
	and bounded changes},
  booktitle = {SIGMOD},
  year = {2013}
}

@INPROCEEDINGS{yan18,
  author = {Cong Yan and Yeye He},
  title = {Synthesizing Type-Detection Logic using Open-source Code},
  booktitle = {SIGMOD},
  year = {2018},
  owner = {yeyehe},
  timestamp = {2018.04.09}
}

@INPROCEEDINGS{yan2018synthesizing,
  author = {Yan, Cong and He, Yeye},
  title = {{Auto-Type: Synthesizing type-detection logic for rich semantic data
	types using open-source code}},
  booktitle = {Proceedings of the 2018 International Conference on Management of
	Data},
  year = {2018},
  organization = {ACM}
}

@INPROCEEDINGS{yu2011,
  author = {Yu, Yang and Heflin, Jeff},
  title = {Extending functional dependency to detect abnormal data in RDF graphs},
  booktitle = {International Semantic Web Conference},
  year = {2011},
  organization = {Springer}
}

@INPROCEEDINGS{zhai2017study,
  author = {Zhai, Chengxiang and Lafferty, John},
  title = {A study of smoothing methods for language models applied to ad hoc
	information retrieval},
  booktitle = {ACM SIGIR Forum},
  year = {2017},
  organization = {ACM}
}

@INPROCEEDINGS{auto-em,
  author = {Chen Zhao and Yeye He},
  title = {{Auto-EM: End-to-end Fuzzy Entity-Matching using Pre-trained Deep
	Models and Transfer Learning}},
  booktitle = {WWW},
  year = {2019}
}

@INPROCEEDINGS{zhao2017controlling,
  author = {Zhao, Zheguang and De Stefani, Lorenzo and Zgraggen, Emanuel and
	Binnig, Carsten and Upfal, Eli and Kraska, Tim},
  title = {Controlling false discoveries during interactive data exploration},
  booktitle = {SIGMOD},
  year = {2017}
}

@ARTICLE{zhou2012scope,
  author = {Zhou, Jingren and Bruno, Nicolas and Wu, Ming-Chuan and Larson, Per-Ake
	and Chaiken, Ronnie and Shakib, Darren},
  title = {SCOPE: parallel databases meet MapReduce},
  journal = {The VLDB Journal},
  year = {2012},
  volume = {21},
  pages = {611--636},
  number = {5},
  publisher = {Springer}
}

@ARTICLE{zhu2017auto,
  author = {Zhu, Erkang and He, Yeye and Chaudhuri, Surajit},
  title = {Auto-join: Joining tables by leveraging transformations},
  journal = {VLDB},
  year = {2017},
  volume = {10},
  number = {10},
  publisher = {VLDB Endowment}
}



@MISC{power-bi-flow,
  title = {{Power BI: Data Flow}},
  howpublished = {\url{https://www.nuget.org/packages/Microsoft.ProgramSynthesis.Extraction.Text/}}
}


@MISC{power-bi-flow,
  title = {{Power BI: Data Flow}},
  howpublished = {\url{https://docs.microsoft.com/en-us/power-bi/transform-model/service-dataflows-create-use}}
}

@MISC{tableau-flow,
  title = {{Tableau: Flow}},
  howpublished = {\url{https://help.tableau.com/current/prep/en-us/prep_build_flow.htm}}
}

@MISC{amazon-workflow,
  title = {{Tableau: Flow}},
  howpublished = {\url{https://aws.amazon.com/blogs/big-data/simplify-data-pipelines-with-aws-glue-automatic-code-generation-and-workflows/}}
}

@MISC{azureml-pipelines,
  title = {{Azure ML: Data Pipelines}},
  howpublished = {\url{https://docs.microsoft.com/en-us/azure/machine-learning/concept-ml-pipelines}}
}

@MISC{ataccama,
  title = {{ataccama: Data Profiling}},
  howpublished = {\url{https://www.ataccama.com/product/data-discovery-and-profiling}}
}

@MISC{Kaggle-Dropbox,
  title = {{Kaggle Expeirment, Shared via Dropbox}},
  howpublished = {\url{https://www.dropbox.com/sh/cfyv5lhzcpiv1xk/AAC5SIKCjuZZL5n5_RKHzMBwa?dl=0}}
}

@article{chaiken2008scope,
  title={SCOPE: easy and efficient parallel processing of massive data sets},
  author={Chaiken, Ronnie and Jenkins, Bob and Larson, Per-{\AA}ke and Ramsey, Bill and Shakib, Darren and Weaver, Simon and Zhou, Jingren},
  journal={Proceedings of the VLDB Endowment},
  volume={1},
  number={2},
  pages={1265--1276},
  year={2008},
  publisher={VLDB Endowment}
}


@incollection{vassiliadis2009near,
  title={Near real time ETL},
  author={Vassiliadis, Panos and Simitsis, Alkis},
  booktitle={New trends in data warehousing and data analysis},
  pages={1--31},
  year={2009},
  publisher={Springer}
}



@MISC{xgboost,
  title = {{XGBoost}},
  howpublished = {\url{https://xgboost.readthedocs.io/en/latest/}}
}



@MISC{BingEntity,
  title = {Bing Entity Search},
  howpublished = {\url{https://azure.microsoft.com/en-us/services/cognitive-services/bing-entity-search-api/}},
  owner = {yeye},
  timestamp = {2017.03.14}
}

@MISC{Deequ,
  title = {{Amazon Deequ Library for Data Validation}},
  howpublished = {\url{https://github.com/awslabs/deequ}}
}

@MISC{DresdenTables,
  title = {{Dresden Web Table Corpus}},
  howpublished = {\url{https://wwwdb.inf.tu-dresden.de/misc/dwtc/}}
}

@MISC{eusprig,
  title = {Spreadsheet mistakes - news stories, compiled by European Spreadsheet
	Risk Interest Group {EuSpRiG}},
  howpublished = {\url{http://www.eusprig.org/horror-stories.htm}},
  owner = {yeyehe},
  timestamp = {2017.09.26}
}

@MISC{frameapi,
  title = {Pandas Data Frame List of APIs},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/frame.html}}
}

@MISC{gartner,
  title = {Self-Service Data Preparation, Worldwide, 2016},
  howpublished = {\url{https://www.gartner.com/doc/3204817/forecast-snapshot-selfservice-data-preparation}},
  owner = {yeyehe},
  timestamp = {2017.03.07}
}

@ARTICLE{gartner17,
  title = {Market Guide for Data Preparation - Gartner, 2017},
  owner = {yeyehe},
  timestamp = {2019.02.14}
}

@MISC{GitHubv3,
  title = {GitHub API},
  howpublished = {\url{https://developer.github.com/v3/}},
  owner = {yeyehe},
  timestamp = {2019.10.21}
}

@MISC{googlewebtables,
  title = {{Google Web Tables}},
  howpublished = {\url{http://research.google.com/tables}}
}

@MISC{groupbyapi,
  title = {Pandas Groupby Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.DataFrame.groupby.html}}
}

@MISC{Informatica,
  title = {{Informatica Rev}},
  howpublished = {\url{https://www.informatica.com/products/data-quality/rev.html}},
  owner = {yeyehe},
  timestamp = {2016.10.21}
}

@Misc{Informatica-DQ-rules,
  title        = {{Informatica Data Quality Rules (Retrieved in 2020-02)}},
  howpublished = {\url{https://www.informatica.com/content/dam/informatica-com/en/collateral/data-sheet/en_informatica-data-quality_data-sheet_6710.pdf}},
}

@MISC{jsonapi,
  title = {Pandas Json Normalize Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.io.json.json_normalize.html}}
}

@MISC{Jupyter,
  title = {Jupyter Notebooks},
  howpublished = {\url{https://jupyter.org/}}
}

@MISC{kaggle,
  title = {Kaggle},
  howpublished = {\url{https://www.kaggle.com/}},
  owner = {yeyehe},
  timestamp = {2019.10.17}
}

@MISC{kaggle-dataset,
  title = {Kaggle Dataset API},
  howpublished = {\url{https://www.kaggle.com/docs/api}{interacting-with-datasets}},
  owner = {yeyehe},
  timestamp = {2019.10.17}
}

@MISC{meltapi,
  title = {Pandas Melt Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.melt.html}}
}

@MISC{mergeapi,
  title = {Pandas Merge Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.merge.html}}
}

@MISC{OpenRefine,
  title = {{OpenRefine (formerly Google Refine)}},
  howpublished = {\url{http://openrefine.org/}}
}

@MISC{paxata,
  title = {Paxata data preparation},
  howpublished = {\url{https://www.paxata.com/}},
  owner = {yeye},
  timestamp = {2017.03.14}
}

@MISC{pivotapi,
  title = {Pandas Pivot Operator API},
  howpublished = {\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.DataFrame.pivot_table.html}}
}

@MISC{PowerBI,
  title = {Power BI},
  howpublished = {\url{https://docs.microsoft.com/en-us/power-bi/desktop-data-types}},
  owner = {yeyehe},
  timestamp = {2017.04.26}
}

@MISC{python-trace,
  title = {{python tracing library}},
  howpublished = {\url{https://pymotw.com/2/trace/}}
}

@MISC{ssis-profiling,
  title = {{SSIS: Data Profiling}},
  howpublished = {\url{https://docs.microsoft.com/en-us/sql/integration-services/control-flow/data-profiling-task?view=sql-server-ver15}}
}

@MISC{TableauPrep,
  title = {Tableau Prep},
  howpublished = {\url{https://www.tableau.com/products/prep}},
  owner = {yeye},
  timestamp = {2017.03.14}
}

@MISC{Talend,
  title = {Talend data validation},
  howpublished = {\url{https://www.talendbyexample.com/talend-data-validation.html}},
  owner = {yeyehe},
  timestamp = {2017.09.28}
}

@MISC{TalendSemantic,
  title = {Talend Data Services Platform Studio User Guide: Semantic Discovery},
  howpublished = {\url{https://help.talend.com/reader/nAXiZW0j0H~2~YApZIsRFw/_u0D0oqWxesgBDSihDgbYA}},
  owner = {yeyehe},
  timestamp = {2018.04.09}
}

@MISC{TFDV,
  title = {{Google TensorFlow Data Validation}},
  howpublished = {\url{https://www.tensorflow.org/tfx/guide/tfdv}}
}

@MISC{Trifacta,
  title = {Trifacta},
  howpublished = {\url{https://www.trifacta.com/}},
  owner = {yeyehe},
  timestamp = {2017.04.26}
}

@MISC{trifacta-profiling,
  title = {{Trifacta: Data Profiling}},
  howpublished = {\url{https://www.trifacta.com/data-profiling/}}
}

@MISC{WebDataCommonsTables,
  title = {{Web Table Corpora from Web Data Commons}},
  howpublished = {\url{http://webdatacommons.org/webtables/}}
}

@MISC{wiktionary,
  title = {Excel error checking rules},
  howpublished = {\url{https://www.wiktionary.org/}},
  owner = {yeyehe},
  timestamp = {2017.09.27}
}

@MISC{word2vec-demo,
  title = {Word embedding demo},
  howpublished = {\url{http://bionlp-www.utu.fi/wv_demo/}},
  owner = {yeyehe},
  timestamp = {2017.04.26}
}

@MISC{word2vec-for-misspellings,
  title = {{Google's trained Word2Vec model }},
  howpublished = {\url{http://mccormickml.com/2016/04/12/googles-pretrained-word2vec-model-in-python/}}
}

@OTHER{,
  owner = {yeyehe},
  timestamp = {2020.03.02}
}

@Article{karp1985fast,
  author    = {Karp, Richard M and Wigderson, Avi},
  title     = {A fast parallel algorithm for the maximal independent set problem},
  journal   = {Journal of the ACM (JACM)},
  year      = {1985},
  volume    = {32},
  number    = {4},
  pages     = {762--773},
  publisher = {ACM New York, NY, USA},
}

@Article{wang1994complexity,
  author  = {Wang, Lusheng and Jiang, Tao},
  title   = {On the complexity of multiple sequence alignment},
  journal = {Journal of computational biology},
  year    = {1994},
  volume  = {1},
  number  = {4},
  pages   = {337--348},
}

@Article{carrillo1988multiple,
  author    = {Carrillo, Humberto and Lipman, David},
  title     = {The multiple sequence alignment problem in biology},
  journal   = {SIAM journal on applied mathematics},
  year      = {1988},
  volume    = {48},
  number    = {5},
  pages     = {1073--1082},
  publisher = {SIAM},
}

@Article{just2001computational,
  author    = {Just, Winfried},
  title     = {Computational complexity of multiple sequence alignment with SP-score},
  journal   = {Journal of computational biology},
  year      = {2001},
  volume    = {8},
  number    = {6},
  pages     = {615--623},
  publisher = {Mary Ann Liebert, Inc.},
}

@Book{cormen2009introduction,
  title     = {Introduction to algorithms},
  publisher = {MIT press},
  year      = {2009},
  author    = {Cormen, Thomas H and Leiserson, Charles E and Rivest, Ronald L and Stein, Clifford},
}

@Misc{enterprise2016trifacta,
  author = {Enterprise, Trifacta Wrangler},
  title  = {Trifacta wrangler (2015)},
  year   = {2016},
}

@Misc{grok,
  title        = {{Grok Patterns}},
  howpublished = {\url{https://github.com/elastic/elasticsearch/blob/master/libs/grok/src/main/resources/patterns/grok-patterns}},
}

@Misc{,
  title        = {{SQL Server SSIS profiling}},
  howpublished = {\url{https://docs.microsoft.com/en-us/sql/integration-services/control-flow/data-profiling-task?view=sql-server-ver15}},
}

@Misc{Glue,
  title        = {{AWS Glue custom classifers}},
  howpublished = {\url{https://docs.aws.amazon.com/glue/latest/dg/custom-classifier.html}},
}

@Misc{xsystem-code,
  title        = {{XSystem Code}},
  howpublished = {\url{https://bitbucket.org/andrewiilyas/xsystem-old/src/outlier-detection/}},
}

@Article{stonebraker2018data,
  author  = {Stonebraker, Michael and Ilyas, Ihab F},
  title   = {Data Integration: The Current Status and the Way Forward.},
  journal = {IEEE Data Eng. Bull.},
  year    = {2018},
  volume  = {41},
  number  = {2},
  pages   = {3--9},
}

@Book{kanji2006,
  title     = {100 statistical tests},
  publisher = {Sage},
  year      = {2006},
  author    = {Kanji, Gopal K},
}

@Article{agresti1992survey,
  author    = {Agresti, Alan and others},
  title     = {A survey of exact inference for contingency tables},
  journal   = {Statistical science},
  year      = {1992},
  volume    = {7},
  number    = {1},
  pages     = {131--153},
  publisher = {Institute of Mathematical Statistics},
}

@InProceedings{hynes2017data,
  author    = {Hynes, Nick and Sculley, D and Terry, Michael},
  title     = {The data linter: Lightweight, automated sanity checking for ml data sets},
  booktitle = {NIPS MLSys Workshop},
  year      = {2017},
}

@Article{naumann2014data,
  author    = {Naumann, Felix},
  title     = {Data profiling revisited},
  journal   = {ACM SIGMOD Record},
  year      = {2014},
  volume    = {42},
  number    = {4},
  pages     = {40--49},
  publisher = {ACM New York, NY, USA},
}

@Misc{msft-ml,
  title        = {{Microsoft ML pipelines}},
  howpublished = {\url{https://www.slideshare.net/KarthikMurugesan2/microsoft-ai-platform-aether-introduction}},
}

@Comment{jabref-meta: databaseType:bibtex;}


==> auto-validate.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Auto-Validate (Basic Version)}

We will start by describing a basic-version of \sj{} for ease of illustration,
before going into more involved
variants of \sj{} that use vertical-cuts (Section~\ref{sec:vertical-cuts})
and horizontal-cuts  (Section~\ref{sec:horizontal-cuts}).

\vspace{-2mm}
\subsection{Preliminary: Pattern Language}
\label{sec:language}
Since we propose to validate data by patterns,
we first briefly describe the pattern language used. 
We note that this is fairly standard (e.g., similar to 
ones used in pattern profiling~\cite{raman2001potter}) 
and not the focus of this work.

Figure~\ref{fig:hierarchy} shows a generalization hierarchy 
used in this work, where leaf-nodes represent the English alphabet, 
and intermediate nodes (e.g., 
\val{<digit>}, \val{<letter>}) represent \textit{token} that values
can generalize into. A pattern is simply a sequence 
of (leaf or intermediate) tokens,
and for a given value $v$, this hierarchy
induces a space of all patterns consistent with $v$, 
denoted by $\mathbf{P}(v)$.
For instance, for a value $v =$ ``\val{9:07}'', we could generate
$\mathbf{P}(v) = $ \{%\val{9:07}, 
%\val{<digit>:07}, 
%\val{9:<digit>\{2\}}, 
 ``\val{<digit>:<digit>\{2\}}'', 
 ``\val{<digit>+:<digit>\{2\}}'', 
 ``\val{<digit>:<digit>+}'', 
 ``\val{<num>:<digit>+}'',  ``\val{9:<digit>\{2\}}'', \ldots
\}, among many other options.

\revised{
Given a column $C$ for which patterns need
to be generated, we define the 
space of \textit{hypothesis-patterns}, 
denoted by $\mathbf{H}(C)$, as the set of non-trivial patterns 
consistent with all values  $v \in C$, or 
$\mathbf{H}(C) = \cap_{v \in C}{\mathbf{P}(v)} \setminus \text{``.*''}$.
Here we make an implicit assumption that values in 
$C$ are homogeneous and drawn from the same domain, which is generally
true for \textit{machine-generated data} in 
enterprise data lakes (e.g., shown in Figure~\ref{fig:domain-example}).
Note that the assumption is used to only simplify our discussion of 
the basic-version of \sj (this section), and will later be relaxed
in more advanced variants (Section~\ref{sec:horizontal-cuts}).
Also note that we explicitly exclude the 
trivial pattern ``.*'' from $\mathbf{H}(C)$,
as it is trivially consistent with $C$.
}


 We call $\mathbf{H}(C)$ hypothesis-patterns, because as we will see 
each $h(C) \in \mathbf{H}(C)$
will be tested like a ``hypothesis'' to determine if $h$ is a good
data-validation pattern.  
(We use $h$ and $h(C)$
interchangeably when the context is clear). 
\begin{example}
\label{ex:patterns}
Given the column $C$ shown in Figure~\ref{fig:generalization},
and the hierarchy in Figure~\ref{fig:hierarchy}, the 
space of hypothesis patterns $\mathbf{H}(C)$ is shown 
at the top of  Figure~\ref{fig:generalization}.
\end{example}

We use an in-house implementation to produce patterns based
on the hierarchy. We emphasize that the
proposed \sj{} framework is not tied to specific 
choices of hierarchy/pattern-languages -- in fact, it is 
entirely orthogonal to such choices, as other variants of languages (e.g., 
Potter's Wheel~\cite{raman2001potter})
are equally applicable in our framework.

\vspace{-2mm}
\subsection{Intuition: Goodness of Patterns}
\label{sec:intuition}
As we alluded to earlier, 
the core challenge in  \sj{} is to determine from 
a large space of patterns
$\mathbf{H}(C)$, whether a
$h(C) \in \mathbf{H}(C)$ is  suitable for data-validation.

Our idea here is to leverage a corpus of 
related tables $\mathbf{T}$ (e.g., drawn from the
same data lake). Intuitively, a pattern
$h(C) \in \mathbf{H}(C)$ is a ``good'' data-validation
pattern for $C$, if it accurately describes the underlying ``domain'' of $C$,
defined as the space of all valid data values.
Conversely, $h(C)$ is a ``bad'' validation pattern, if:
\begin{itemize}[leftmargin=*,topsep=0pt]
\item[](1) $h(C)$ does not capture all valid values that can be
generated for the underlying ``domain'' of $C$;
\item[](2) $h(C)$ does not produce sufficient matches in $\mathbf{T}$.
\end{itemize}

Both of these are reasonable requirements -- 
(1) is intuitive, because as discussed the danger in
data-validation is to produce
patterns that only cover a subset of valid values in that domain, 
resulting in false-positive detection.
Requirement (2) is also sensible, because we want to see sufficient
evidence in $\mathbf{T}$ 
before declaring a pattern $h(C)$ to be a common ``domain''
of interest (it would not be reliable if
we can only find one or two columns in $\mathbf{T}$ matching $h(C)$).


We note that both of these two requirements can be reliably tested using 
$\mathbf{T}$ alone and without involving humans.
Testing (2) is straightforward with standard regex matches. 
Testing (1) is also feasible,
under the assumption that most data columns 
in $D \in \mathbf{T}$ contain homogeneous
values drawn from the same underlying 
domain, which is generally true for production data
in enterprise data lakes that are typically
``machine-generated''.
(Homogeneity is less likely to hold on data
produced by other means, e.g., manually entered by human operators).

Before we show how to test 
requirement (1) using data columns 
$D \in \mathbf{T}$,
we would like to highlight the fact that
we are now dealing with two types of columns that
can be a bit confusing --
the first is the input column $C$ for which we need to
generate validation patterns $h$, and the second is 
columns $D \in \mathbf{T}$ from which we draw evidence 
to determine the goodness of $h$.
To avoid confusion,  we will follow the standard of referring
to the first as the \textit{query column}, denoted by $C$,
and the second as \textit{data columns}, denoted by $D$.


\begin{figure*}
\vspace{-19mm}
        \centering
        \includegraphics[width=0.95\textwidth]{figures/intuition.png}
\caption{Leverage corpus $\mathbf{T}$ to determine ``good'' vs. ``bad'' hypothesis patterns, for a given query column $C$.}
\vspace{-3mm}
\label{fig:intuition}
\end{figure*}


We now show how to test requirement (1) using $\mathbf{T}$ below.

\begin{example}
\label{ex:intuition} 
The left of
Figure~\ref{fig:intuition} shows a query column $C$ for which
validation patterns need to be generated. A few
hypothesis-patterns in $\mathbf{H}(C)$ are listed in
the middle of the figure. In this example, we intuitively know
that $h_1(C)$ and $h_2(C)$ are ``bad'' patterns
since they 
are too ``narrow'' and would lead to false-alarms,
while $h_5(C)$ is a ``good'' validation pattern
that suitably generalizes the underlying domain. 

We show that such determinations can 
be inferred using $\mathbf{T}$.
Specifically, $h_1(C)$ is a ``bad'' pattern based on $\mathbf{T}$,
because we can find many columns like $D \in \mathbf{T}$ 
shown on the right of Figure~\ref{fig:intuition}
that are ``impure'' -- these columns contain
values that match $h_1(C)$, as well as values that do not
(e.g., ``{\small \texttt{9/12/2019 12:01:32 PM}}'',
where the ``{\small \texttt{PM}}'' part does not match $h_1(C)$).
A large number of ``impure'' columns like this would
indicate that $h_1(C)$ is a not a good pattern to describe 
the underlying domain, 
because if it were, we should not see
many impure columns like $D \in \mathbf{T}$ given homogeneity.

Similarly, we can show that $h_2(C)$ is not a good validation pattern,
for using $h_2(C)$ to describe the 
domain would again make many columns like $D$ ``impure'' 
(values like ``\val{10:02:20 AM}'' are inconsistent
with $h_2(C)$ since they have two-digit hours, whereas
$h_2(C)$ uses a single \val{<digit>} for hours),
  suggesting that $h_2(C)$ may again be too narrow.

Using $h_5(C)$ to describe the domain, 
on the other hand, would not yield many
``impure'' columns in $\mathbf{T}$, suggesting that it
may be a good validation pattern.
\end{example}



Intuitively, we can use the \textit{impurity} of 
data columns $D \in \mathbf{T}$ 
relative to a pattern $h$,
to infer whether $h$ is a good validation pattern
for the domain, defined as follows.
\begin{definition}
\label{def:impurity}
The \textit{impurity} of a data column 
$D \in \mathbf{T}$, relative to a given hypothesis pattern $h$,
is defined as:
\begin{equation}
\label{eqn:impurity}
\text{Imp}_{D}(h) = \frac{|\{v | v \in D, h \notin \mathbf{P}(v)\}|}{|\{ v | v \in D \}|}
\end{equation}
\end{definition}

This definition is intuitive -- we measure 
impurity as the fraction 
of values in $D$ not matching $h$.



\begin{example}
\label{ex:fpr}
In Figure~\ref{fig:intuition}, 
$\text{Imp}_D(h_1)$ can be calculated as $\frac{2}{12}$,
since the last 2 values (with ``\val{PM}'') 
out of 12 do not match $h_1$.

Similarly, $\text{Imp}_D(h_2)$ can be calculated as $\frac{8}{12}$,
since the last 8 values in $D$ (with two-digit hours) 
do not match $h_2$.

Finally, $\text{Imp}_D(h_5)$ is $\frac{0}{12}$,
since all values in $D$ match $h_5$.
\end{example}



We note that if $h(C)$ is used to validate
a data column $D$ (in the same domain as $C$)
arriving in the future, then 
Imp$_D(h)$ directly corresponds to
expected false-positive-rate (FPR):

\begin{definition}
\label{def:fpr}
The expected \textit{false-positive-rate} (FPR) of using pattern $h(C)$ 
to validate a data column $D$ drawn from the same domain as $C$,
denoted by $\text{FPR}_{D}(h)$, is defined as:
\begin{equation}
\label{eqn:fpr}
\text{FPR}_{D}(h) = \frac{\text{FP}_{D}(h)}{\text{TN}_{D}(h)+\text{FP}_{D}(h)}
\end{equation}
Where FP$_{D}(h)$ and TN$_{D}(h)$ are the number of 
false-positive detection and true-negative detection of $h$ on $D$,
respectively. 
\end{definition}
Note that since $D$ is from the same domain as $C$,
ensuring that TN$_{D}(h)$ + FP$_{D}(h)$ = $|D|$, 
$\text{FPR}_{D}(h)$ can be rewritten as:
\begin{equation}
\label{eqn:fpr}
\text{FPR}_{D}(h) = \frac{|\{v | v \in D, h \notin \mathbf{P}(v)\}|}{|\{v | v \in D \}|} = \text{Imp}_D(h)
\end{equation}
Thus allowing us to estimate $\text{FPR}_{D}(h)$ using $\text{Imp}_D(h)$.

\begin{example}
\label{ex:fpr-impurity}
Continue with Example~\ref{ex:fpr}, it can be
verified that the expected 
FPR of using $h$ as the validation pattern for $D$,
directly corresponds to the impurity $\text{Imp}_D(h)$ --
e.g., using $h_1$ to validate $D$ has $\text{FPR}_{D}(h_1)$
= $\text{Imp}_D(h_1)$ = $\frac{2}{12}$; while using 
$h_5$ to validate $D$ has $\text{FPR}_{D}(h_5) = \text{Imp}_D(h_5) = 0$, etc.
\end{example}

Based on FPR$_{D}(h)$ defined for one column $D \in \mathbf{T}$, 
we can in turn define the estimated FPR on the entire corpus $\mathbf{T}$,
using all column $D \in \mathbf{T}$ 
where some value $v \in D$ matches $h$:
\begin{definition}
\label{def:fpr_corpus}
Given a corpus $\mathbf{T}$, we estimate the 
FPR of pattern $h$ on  $\mathbf{T}$, 
denoted by FPR$_{\mathbf{T}}(h)$, as:
\begin{equation}
\label{eqn:fpr_agg}
\text{FPR}_{\mathbf{T}}(h) = \avg_{D \in \mathbf{T}, v \in D, h \in \mathbf{P}(v) }{\text{FPR}_{D}(h)}
\end{equation} 
\end{definition}
%Note that $\text{FPR}_{\mathbf{T}}(h)$ uses
%all column $D \in \mathbf{T}$ where some value $v \in D$ 
%match $h$, or written as $h \in \mathbf{P}(v)$.

%This is consistent with our homogeneity assumption 
%of machine-generated data --
%because values in $D$ are generated by the same program
%and thus drawn from the same domain, 
%the fact that $v \in D$ matches a domain pattern $h$ 
%indicates that $D$ is from the same domain described by $h$,
%allowing us to use $\text{FPR}_{D}(h)$ as a piece of local evidence
%to estimate $h$.

\begin{example}
\label{ex:fpr_t}
Continue with the $h_5$ in Example~\ref{ex:fpr}
and Example~\ref{ex:fpr-impurity}. Suppose 
there are 5000 data columns $D \in \mathbf{T}$ 
where some value $v \in D$ matches $h_5$.
Suppose 4800 columns out of the 5000 have $\text{FPR}_{D}(h_5) = 0$, 
and the remaining 200 columns have $\text{FPR}_{D}(h_5) = 1\%$. 
The overall $\text{FPR}_{\mathbf{T}}(h_5)$ 
can be calculated as $\frac{200 * 1\%}{5000} = 0.04\%$,
using Equation~\eqref{eqn:fpr_agg}.
\end{example}



We emphasize that a low FPR is 
critical for data-validation, because given a large 
number of columns and values in production 
data, even a 1\% FPR
can translate into many false-alarms, 
all of which require human
attention to resolve.
FPR is thus a key objective we minimize in \sj.


\vspace{-2mm}
\subsection{Problem Statement}
We now describe the basic version 
of \sj{} as follows. 
Given an input query column $C$ and a background corpus $\mathbf{T}$,
we need to produce a validation pattern $h(C)$, 
such that $h(C)$ is expected to have a low FPR
but can still catch many quality issues.
We formulate this as an optimization problem.
Specifically, we introduce an FPR-Minimizing 
version of Data-Validation (FMDV), defined as:
\begin{align}
\hspace{-1cm} \text{(FMDV)} \qquad{} \min_{h \in \mathbf{H}(C)} & \text{FPR}_\mathbf{T}(h)   \label{eqn:fmdv_obj} \\ 
 \mbox{s.t.} ~~ & \text{FPR}_\mathbf{T}(h) \leq r \label{eqn:fmdv_fpr} \\
 & \text{Cov}_\mathbf{T}(h) \geq m \label{eqn:fmdv_cov}
\end{align}
Where $\text{FPR}_\mathbf{T}(h)$ is the 
expected FPR of $h$ estimated using $\mathbf{T}$,
which has to be lower than a given target threshold $r$
(Equation~\eqref{eqn:fmdv_fpr}); and
$\text{Cov}_\mathbf{T}(h)$ is the coverage of $h$, or 
the number of columns in $\mathbf{T}$ that match $h$,
which has to be greater than a given threshold 
$m$ (Equation~\eqref{eqn:fmdv_cov}). Note that
these two constraints directly map to the 
two ``goodness'' criteria in Section~\ref{sec:intuition}.

The validation pattern $h$ we produce for $C$ is
then the minimizer
of FMDV from the hypothesis space 
$\mathbf{H}(C)$ (Equation~\eqref{eqn:fmdv_obj}).
We note that this can be interpreted as a conservative approach to
data-validation -- our goal is
to find a ``safe'' pattern $h(C)$ with minimum FPR.

%ensures that the FPR is below
%a predefined target threshold $r$ (e.g., 1\% FPR would correspond
%to a target precision of 99\%), or otherwise we do not consider
%the solution to be feasible and do not produce a validation pattern.
%The second constraint in 
%ensures that the coverage of pattern $h(C)$ on $\mathbf{T}$
%is significant (e.g., $m$ = 1000, meaning that there are at least
%1000 columns in $\mathbf{T}$ matching this pattern), for otherwise
%this pattern $h(C)$ does not have sufficient representation in
%$\mathbf{T}$ for us to draw reliable conclusions, and furthermore
%if $h(C)$ only occurs once or twice it is unlikely to be a commonly
%used data-format for us to declare this to be a ``domain'' of data values.

%revised
\iftoggle{fullversion}{
\begin{example}
\label{ex:fmdv}
Continue with Example~\ref{ex:fpr_t}.
Suppose we have FMDV with a target FPR rate $r$ no greater
than $0.1\%$, and a required coverage of at least $m = 100$.
Given the 3 example hypothesis patterns in Figure~\ref{fig:intuition},
we can see that patterns $h_1$ and $h_2$ are not feasible solutions
because of their high estimated FPR.
Pattern $h_5$ has an estimated FPR of 0.04\% and a coverage of 5000,
and is thus a possible solution to FMDV.
\end{example}
} %iftoggle


\iftoggle{fullversion}{
\revised{
\begin{lemma}
\label{lem:fmdv}
In a simplified scenario, where each column corresponds to 
one domain, which in turn corresponds to one regex
pattern. Assuming that values in a column are sampled at
random from the underlying domain. Given a query column $Q$,
and a corpus with a large number of 
columns drawn from the underlying domain of $Q$, 
asymptotically the optimal solution of FMDV 
for $Q$ (with $r=0$) converges to the domain pattern of $Q$ with high probability.
\end{lemma}

This result assumes a simplified scenario, where
each column corresponds to one domain, and each 
domain corresponds to a regex pattern. Values in a column
corresponding are generated
by sampling from the underlying
domain/pattern. Given a sufficiently large number of columns in
data corpus, asymptotically any candidate patterns 
that ``under-generalizes'' the
domain will be pruned away because of FPR violations, 
leaving the latent domain pattern to be the optimal solution.

While this simplified analysis would not extend to the general case
in practice (because noise can be introduced via different generative
processes that are unknown, and are only modeled 
via an FPR constraint), we believe
this nevertheless shows that our formulation is a principled
attempt at solving the problem in question. Extending the formulation
to consider/model noises in data sets would be interesting
directions of future work.
}
}


%\revised
\iftoggle{fullversion}
{
We explored alternative formulations, such as 
coverage-minimizing data-validation (CMDV), where
we minimize coverage $\text{Cov}_\mathbf{T}(h)$
in the objective function in place of FPR$_\mathbf{T}(h)$ as in FMDV.
%The intuition here is that patterns with
%smaller coverage on $\mathbf{T}$ are more precise/restrictive
%and may catch more quality issues.
%\begin{align}
%\hspace{-1cm} \text{(CMDV)} \qquad{} \min_{h \in \mathbf{H}(C)} & \text{Cov}_\mathbf{T}(h)   \label{eqn:cmdv_obj} \\ 
% \mbox{s.t.} ~~ & \text{FPR}_\mathbf{T}(h) \leq r \label{eqn:cmdv_fpr} \\
% & \text{Cov}_\mathbf{T}(h) \geq m \label{eqn:cmdv_cov}
%\end{align}
We omit details in the interest of space, 
but will report that the conservative FMDV is more
effective in practice (as CMDV tends to under-generalize).
}
%\revised



\vspace{-2mm}
\subsection{System Architecture}
\label{sec:architecture}
While FMDV is simple overall, 
a naive implementation would
require a full scan of $\mathbf{T}$ in order to compute  
$\text{FPR}_\mathbf{T}(h)$ and $\text{Cov}_\mathbf{T}(h)$ for each
hypothesis $h$.
This is both costly and slow
considering the fact that  $\mathbf{T}$ is typically large 
in enterprise data lakes (e.g., in terabytes), 
where a full-scan can take hours. 
This is especially problematic for user-in-the-loop 
validation such as Google's TFDV, where users
are expected to review/modify suggested validation rules --
having users wait for hours is clearly not an option. 

We thus build an offline index that has summary
statistics of $\mathbf{T}$,  so that at online time and given a new 
query column $C$, 
we can evaluate hypothesis patterns $h$ efficiently using only the index, 
without needing to scan $\mathbf{T}$ again.

The architecture of our system can be
seen in Figure~\ref{fig:architecture}. 

\textbf{Offline stage.}
In the offline stage, we perform
one full scan of $\mathbf{T}$, enumerating all possible patterns for
each $D \in \mathbf{T}$ as 
$\mathbf{P}(D) = \cup_{v \in D} \mathbf{P}(v)$,
or the union of patterns for all $v \in D$
(where $\mathbf{P}$ is the generalization hierarchy 
in Section~\ref{sec:language}).
%that can ``cover'' a substantial fraction $\theta$ (e.g., 50\%) of values in 

\revised{
Note that the space of $\mathbf{P}(D)$ 
can be quite large, especially for
``wide'' columns with many tokens like discussed in Figure~\ref{fig:generalization}. 
In practice and to limit $\mathbf{P}(D)$, 
we produce $\mathbf{P}(D)$ as 
$\cup_{v \in D, t(v)<\tau} \mathbf{P}(v)$, where $t(v)$ is the number
of tokens in $v$ (defined as the number of consecutive sequences
of letters, digits, or symbols in $v$), 
and $\tau$ is some fixed constant (e.g., 8 or 13) to make $\mathbf{P}(D)$
tractable.  Leveraging the observation that
such wide columns typically have composite structures 
concatenated from multiple sub-domains, we will describe
a vertical-cut technique (Section~\ref{sec:vertical-cuts}), to ensure that
wide columns can be safely skipped in offline 
indexing without affecting result quality.
%(e.g., Figure~\ref{fig:generalization}
%can be decomposed into a date and a time-stamp).
}


For each pattern $p \in \mathbf{P}(D)$,
we pre-compute the local impurity score of $p$ on 
$D$ as $\text{Imp}_{D}(p)$,
since $p$ may be hypothesized 
as a domain pattern for some query column $C$ in the future,
for which this $D$ can provide a piece of local evidence.
%Recall that $\text{Imp}(D, p)$ directly corresponds to 
%$\text{FPR}_{D}(p)$ (Definition~\ref{def:fpr}), providing
%a piece of local evidence on the goodness of $p$.

Let $\mathbf{P}(\mathbf{T}) = \{p | p \in \mathbf{P}(D), D \in \mathbf{T}\}$
be the space of possible patterns in $\mathbf{T}$.
We pre-compute $\text{FPR}_{\mathbf{T}}(p)$ for
all possible $p \in \mathbf{P}(\mathbf{T})$
on the entire $\mathbf{T}$, 
by aggregating local $\text{Imp}_{D}(p)$ scores using
Equation~\eqref{eqn:fpr} and~\eqref{eqn:fpr_agg}.
The coverage scores $\text{Cov}_{\mathbf{T}}(p)$ of all $p$ can be 
pre-computed similarly as 
$\text{Cov}_{\mathbf{T}}(p) = |\{ D | D \in \mathbf{T}, v \in D, p \in \mathbf{P}(v) \}|$.

The offline index we build can then be used to lookup,
for each possible $p \in \mathbf{P}(\mathbf{T})$, its 
pre-computed $\text{FPR}_{\mathbf{T}}(p)$ 
and $\text{Cov}_{\mathbf{T}}(p)$ scores.
We note that this pattern-to-score index is 
orders of magnitude smaller than the original
$\mathbf{T}$ -- e.g., a 1TB corpus $\mathbf{T}$ 
yields an index less than 1GB in our test.


\textbf{Online stage.}
At online query time, for a given
query column $C$, we enumerate $h \in \mathbf{H}(C)$,
and use the offline index to perform a lookup to retrieve 
$\text{FPR}_{\mathbf{T}}(p)$ and $\text{Cov}_{\mathbf{T}}(p)$
scores for FMDV, without needing to scan the full $\mathbf{T}$ again.
This indexing approach reduces our latency per 
query-column $C$ from hours to
tens of milliseconds, which makes it possible
to do interactive, human-in-the-loop
verification of suggested rules,
as we will report in experiments.


\begin{figure}[t]
\vspace{-2mm}
        \centering
        \includegraphics[width=0.5\textwidth]{figures/architecture.png}
\caption{Architecture of the \sj{} System.}
\label{fig:architecture}
\end{figure}



















